Every Bit Counts in Consensus

Consensus enables n processes to agree on a common valid L-bit value, despite t < n/3 processes being faulty and acting arbitrarily. A long line of work has been dedicated to improving the worst-case communication complexity of consensus in partial synchrony. This has recently culminated in the worst-case word complexity of O(n^2). However, the worst-case bit complexity of the best solution is still O(n^2 L + n^2 kappa) (where kappa is the security parameter), far from the \Omega(n L + n^2) lower bound. The gap is significant given the practical use of consensus primitives, where values typically consist of batches of large size (L > n). This paper shows how to narrow the aforementioned gap while achieving optimal linear latency. Namely, we present a new algorithm, DARE (Disperse, Agree, REtrieve), that improves upon the O(n^2 L) term via a novel dispersal primitive. DARE achieves O(n^{1.5} L + n^{2.5} kappa) bit complexity, an effective sqrt{n}-factor improvement over the state-of-the-art (when L > n kappa). Moreover, we show that employing heavier cryptographic primitives, namely STARK proofs, allows us to devise DARE-Stark, a version of DARE which achieves the near-optimal bit complexity of O(n L + n^2 poly(kappa)). Both DARE and DARE-Stark achieve optimal O(n) latency.

==> sections/curse_of_GST.tex <==
\section{The curse of GST}

In this section, we show that any \emph{naive} partially-synchronous algorithm such that ensuring that (i) every-correct process observes a message $m$ implies (ii) $m$ has been broadcasted by some process necessarily suffers from a worst case communication complexity of $\Omega((t+1) \cdot n \cdot |m| $.

Each process $p \in \Psi$ is assigned a \emph{protocol} $\Pi_p$ to follow.
Formally, a protocol $\Pi_p$ is a tuple $(\mathcal{S}_p, s_0^p, \mathcal{M}_p, \mathcal{I}_p, \mathcal{O}_p, \mathcal{T}_p)$, where $\mathcal{S}_p$ represents a set of states $p$ can take,\footnote{We refer to $\mathcal{S}_p$ as the \emph{state set} of $\Pi_p$.} $s_0^p \in \mathcal{S}_p$ is the initial state of $p$, $\mathcal{M}_p$ is a set of messages $p$ can send or receive, $\mathcal{I}_p$ is a set of internal events $p$ can observe, $\mathcal{O}_p$ is a set of internal events $p$ can produce and $\mathcal{T}_p: \mathcal{S}_p \times P(\mathcal{M}_p \cup \mathcal{I}_p) \to \mathcal{S}_p \times P(\mathcal{M}_p \cup \mathcal{O}_p)$ maps a state and a set of received messages and observed internal events into a new state and a set of sent messages and produced internal events.\footnote{We denote by $P(X)$ the power set of $X$.}

Processes can forward messages to other processes, they can include messages in other messages they send, and we assume that an included or forwarded message can still be authenticated.
Each message $m$ has a unique sender $\mathit{sender}(m) \in \Psi$ and a unique receiver $\mathit{receiver}(m) \in \Psi$.
Finally, we assume a computationally bounded adversary, i.e., signatures of processes that follow their protocol \emph{cannot} be forged.

\paragraph{Events, executions \& behaviors}
We define an \emph{event} as a tuple $(p, I, O, \tau)$, where $p \in \Psi$ is a process on which the event occurs, $I$ represents a finite set of received messages and observed internal events,$O$ represents a finite set of sent messages and produced internal events\footnote{Observe the difference between events and internal events.}, and $\tau$ represents the time when the event occurs according to some global clock\footnote{This global clock is a priori non-accessible by the correct processes}.
An \emph{execution} is a well-formed sequence of events: (1) every received message was previously sent, (2) if the execution is infinite, every sent message is received, and (3) if an event $(p, I, O, \tau)$ precedes another event $(p', I', O', \tau')$, then $\tau \leq \tau'$.
Similarly, a \emph{behavior} is a well-formed sequence of events: (1) all events occur on the same process $p \in \Psi$, (2) if a message $m$ with $\mathit{sender}(m) = p$ is received in the behavior, then the message was previously sent in the behavior, and (3) if the behavior is infinite, every message $m$ with $\mathit{receiver}(m) = p$ which is sent in the behavior is received in the behavior.

Given an execution $\alpha$, $\alpha|_p$ denotes the sequence of events in $\alpha$ associated with a process $p \in \Psi$ (i.e., the behavior of $p$ given $\alpha$). 

A behavior $\beta_p = (p, I_1, O_1, \tau_1), (p, I_2, O_2, \tau_2), ...$ is \emph{valid} according to $\Pi_p$ if and only if it conforms to the assigned protocol $\Pi_p$, i.e., if and only if there exists a sequence of states $s_0, s_1, ...$ in $\mathcal{S}_p$ such that $s_0 = s_0^p$ and, for all $i \geq 1$, $\mathcal{T}_p(s_{i - 1}, I_i) = (s_i, O_i)$.
For every behavior $\beta$, we define $\mathit{sent}(\beta)$ (resp., $\mathit{received}(\beta)$) to be the set of sent (resp., received) messages in $\beta$.

Finally, for every message $m$, we assume that there exists a valid behavior of $\mathit{sender}(m)$ in which $m$ is sent.

\paragraph{Distributed protocols}
A tuple $\Pi = (\Pi_p, \Pi_q, ..., \Pi_z)$, where $\Psi = \{p, q, ..., z\}$, is a \emph{distributed protocol}.
We assume that sets of messages each process can send or receive are identical (i.e., $\mathcal{M}_p = \mathcal{M}_q$, for all $p, q \in \Psi$); we denote this set of messages by $\mathcal{M}$.

A process $p$ is \emph{correct} in an execution $\alpha$ according to $\Pi = (\Pi_p, \Pi_q, ..., \Pi_z)$ if and only if $\alpha|_p$ is valid according to $\Pi_p$.

Otherwise, $p$ is \emph{faulty} in $\alpha$ according to $\Pi$.
If a process is correct in an infinite execution, then infinitely many events occur on the process (i.e., a process correct in an infinite execution is \emph{live}).
We denote by $\mathit{Corr}_{\Pi}(\alpha)$ the set of processes correct in execution $\alpha$ according to $\Pi$.
Whenever we say that ``$\alpha$ is an execution of a distributed protocol $\Pi$'', we mean that each process is considered correct or faulty in $\alpha$ according to $\Pi$.
The set of all possible executions of a distributed protocol $\Pi$ is denoted by $\mathit{execs}(\Pi)$.


\paragraph{Communication network}
We assume that the communication network is fully-connected and reliable, i.e., correct processes are able to communicate among themselves.
Furthermore, we assume that the network is either asynchronous or partially synchronous~\cite{DLS88}.

==> sections/discussion.tex <==
\section{Discussion}

\subsection{Obtaining Strong Validity with quadratic communication}

The actual \name protocol only ensures weak validity (if all processes are correct and a process decides $w$, then $w$ is proposed by a correct process) but does not ensure \emph{strong validity}: If all correct processes propose the same value $w$, then $w$ is decided. In this subsection, we add a groundwork step before \name to obtain \namebis that ensures strong validity.

We assume another $(k', n)$-threshold signature scheme~\cite{LJY16}, where $k' = f + 1$ (and not $2f+1$). In the remaining, \name is used in a black-box fashion, so we use the same names $ShareSign$, $ShareVerify$, $Combine$, $Verify$ for the $(k', n)$-threshold signature without fearing any ambiguity with the $(2f+1, n)$-threshold signature used in \name.

 The basic idea is to propose and accept only values that are \emph{legitimate}, in the sense that deciding one of them cannot violate strong validity. Hence a groundwork is added to know what are the legitimate values. At first round of the groundwork, every correct process send its (signed) proposal. If a process $p$ does not receive $f+1$ times the same proposal, it knows that any value $w$ could be decided safely. A naive solution could consist in broadcasting $2f+1$ signed proposals, s. t. eventually, every correct process knows that any value $w$ could be decided safely. But it would induce a $O(n^3)$ communication complexity. We adapt this idea with some optimization to reach a $O(n^2)$ communication complexity. The groundwork pseudo-code is presented in \ref{algorithm:groundwork} and counts 3 rounds that are presented here.
 \begin{enumerate}
     \item PROPOSAL: every process $i$ send its partially-signed proposal $[PROPOSAL, proposal_i]_{\sigma_i}$ (line \ref{line-gw:bcast-proposal}).
     
     \item ECHO: Upon the reception of $2f+1$ proposals (line \ref{line-gw:proposal-reception}), a process deals with two possible situations:
     \begin{enumerate}
         \item It did not receive more than $f$ times the same proposal (line \ref{line-gw:not-same-proposals}). It knows that any value can be safely decided. To inform other processes, it broadcasts a message $[ECHO, \bot]_{\sigma_i}$ (line \ref{line-gw:claim-not-same-proposals} and \ref{line-gw:bcast-echo}).
         
         \item It received $f+1$ times the same proposal $w$ (line \ref{line-gw:same-proposals}). Potentially, it could be the only legitimate  value to decide. To inform the other processes, it broadcast a message $[ECHO, \sigma]$ where $\sigma$ is the $(f+1)$-threshold signature of message $[PROPOSAL, w]$ (line \ref{line-gw:certify-same-proposals} and \ref{line-gw:bcast-echo}). 
          \end{enumerate}
     
     \item JUSTIFICATION: Upon the reception of $2f+1$ echo messages, a process deals with two possible situations:
     \begin{enumerate}
     \item It receives $f+1$ messages of the form $[ECHO, \bot]_{\sigma_j}$ (line \ref{line-gw:uniform-claim-not-same-proposals}).
     The process knows
     that any value can be safely decided, but now, it can prove it with a reasonable cost. To inform other processes, it broadcasts a message $[JUSTIFICATION, \sigma]$ where $\sigma$
 is the $(f+1)$-threshold signature of message $[ECHO, \bot]$ (line \ref{line-gw:certify-uniform-claim-not-same-proposals} and \ref{line-gw:bcast-justification}). 
 
 \item It does not receive $f+1$ messages of the form $[ECHO, \bot]_{\sigma_j}$. Here again, two possibilities: 
 \begin{enumerate}
     \item it receives $m_x = [ECHO, \sigma_x]$ and $m_y = [ECHO, \sigma_y]$ that justifies two different values $x$ and $y$ (line \ref{line-gw:at-least-two-different proposals}). Since at least two different correct processes proposed two different values, the process knows
     that any value can be safely decided, but now, it can prove it with a reasonable cost. To inform other processes, it broadcasts $[JUSTIFICATION, (m_x, m_y)]$ (line \ref{line-gw:certify-at-least-two-different-proposals} and \ref{line-gw:bcast-justification-2}).
     \item it receives only message of the form $m_w = [ECHO, \sigma_w]$ that justifies $w$ ($Verify([PROPOSAL,w], \sigma_w)$) (line \ref{line-gw:all-processes-consider-value-legitimate}). In that case, all the correct processes also receive $[ECHO, \sigma_w]$ and thus knows that $w$ can be decided safely. Moreover, it updates its proposal to $w$ before starting \name (line \ref{line-gw:update-proposal-upon-same-proposals}). 
 \end{enumerate}
     \end{enumerate}
     
     \item Later, a message $m$ legitimates a value $w$ iff it is a well-formed JUSTIFICATION message or if $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$. %either (1)  $m = (JUSTIFICATION, \sigma)$ with $Verify([ECHO, \bot], \sigma)$ or 
 %(2)  $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$ or
 %(3) $m = ( JUSTIFICATION, \{m_x, m_y\} )$ with $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ and $x \neq y$. 
 Upon the reception of the first JUSTIFICATION message, it is broadcast in order to ensure uniformity, i. e. if a value is considered legitimate by a correct process, it is considered legitimate by all correct processes by time $GST + \delta$.
     It is worthy to note that if no justification message is sent by a correct process, it means it is in case 3) b) ii) which means that every correct process receives a message $[ECHO, \sigma_w]$  s.t. $Verify([PROPOSAL, w], \sigma_w)$.
 \end{enumerate}
 
 The pseudo-code of \namebis is presented in algorithms \ref{algorithm:groundwork} and \ref{algorithm:wrapper-for-strong-validity}.

\begin{algorithm} 
\caption{GroundWork: Pseudocode for process $P_i$}
\label{algorithm:groundwork}
\begin{algorithmic} [1]

%Sending Phase proposal
\State \textbf{upon} \texttt{start}: \Comment{start of the algorithm}

\State \hskip2em $certified \gets \emptyset$

\medskip

\State \hskip2em $m^p.\mathit{type} \gets PROPOSAL$
\State \hskip2em $m^p.\mathit{proposal} \gets proposal_i$
\State \hskip2em $m^p.\mathit{partial\_sig} \gets \mathit{ShareSign}_i([m^p.\mathit{type}, m^p.\mathit{proposal}])$
\State \hskip2em \texttt{broadcast} $m^p$ \label{line-gw:bcast-proposal}

\medskip

%%%Rcving Phase proposal
\State \hskip2em \textbf{wait for } $2f + 1$ proposals: $M \gets \{m'|m'.type = PROPOSAL\}$.  \label{line-gw:proposal-reception}
\State \hskip2em \textbf{if } $\exists M' \subset M$, s. t. $\forall m', m'' \in M', m'.\mathit{proposal} = m''.proposal$: \label{line-gw:same-proposals}

\State \hskip4em $m^e.\mathit{cert} \gets Combine(\{m'.\mathit{partial\_sig}| m' \in M'\})$ \label{line-gw:certify-same-proposals}
%\State \hskip4em $proposal_i \gets w$ where $Verify([Proposal, w], m^e.\mathit{cert})$ \label{line-gw:update-proposal-upon-same-proposals}
\State \hskip2em \textbf{else } \label{line-gw:not-same-proposals} 
\State \hskip4em $m^e.\mathit{cert} \gets \bot$ \label{line-gw:claim-not-same-proposals}

\State \hskip2em $m^e.\mathit{type} \gets ECHO$
\State \hskip2em $m^e.\mathit{partial\_sig} \gets ShareSign_i([m^e.\mathit{type}, m^e.\mathit{cert}])$

\State \hskip2em \texttt{broadcast} $m^e$ \label{line-gw:bcast-echo}

\medskip
%%%
\State \hskip2em \textbf{wait for } $2f + 1$ echo messages: $M \gets \{m'|m'.type = ECHO\}$.
\State \hskip2em \textbf{if } $\exists M' \subset M$, s. t. $\forall m' \in M', m'.\mathit{cert} = \bot$: \label{line-gw:uniform-claim-not-same-proposals}

\State \hskip4em $m^j.\mathit{type} \gets$ $JUSTIFICATION$

\State \hskip4em $m^j.\mathit{justification} \gets$ $Combine(\{m'.\mathit{partial\_sig}| m' \in M'\})$ \label{line-gw:certify-uniform-claim-not-same-proposals}

\State \hskip4em \texttt{broadcast} $m^j$ \label{line-gw:bcast-justification}

\State \hskip2em \textbf{else if}: $\exists m_x, m_y \in M$ s. t. $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ with $x \neq y$ \label{line-gw:at-least-two-different proposals}

\State \hskip4em $m^j.\mathit{type} \gets$ $JUSTIFICATION$

\State \hskip4em $m^j.\mathit{justification} \gets$ $\{m_x, m_y\}$ \label{line-gw:certify-at-least-two-different-proposals}

\State \hskip4em \texttt{broadcast} $m^j$ \label{line-gw:bcast-justification-2}


\State \hskip2em \textbf{else}: \label{line-gw:all-processes-consider-value-legitimate}

\State \hskip4em $proposal_i \gets w$ where  $Verify([PROPOSAL, w], m'.cert)$ for some $m' \in M$ \label{line-gw:update-proposal-upon-same-proposals}

\State \hskip2em \textbf{trigger} \texttt{terminate\_GroundWork}

\medskip

%%%Uniformity Phase
\State \textbf{upon} first reception of a message $m$ with $m.type = JUSTIFICATION$
\State \hskip2em \texttt{broadcast} $m$ if it is not already done \label{line-gw:forward-justification}

%\medskip

%\State \textbf{upon} reception of a message $m$ with $m.type = ECHO$ and $Verify([ECHO, x], m.cert)$
%\State \hskip2em $certified \gets certified \cup \{x\}$
%\State \hskip2em \textbf{if} $|certified| \leq 2$:
%\State \hskip4em \texttt{broadcast} $m$

\medskip
%Utility

\State \textbf{function} \texttt{legitimate}(\texttt{Message} $m$, \texttt{Integer} $w$):
\State \hskip2em \textbf{if} either
\State \hskip4em (1)  $m = (JUSTIFICATION, \sigma)$ with $Verify([ECHO, \bot], \sigma)$ or 
\State \hskip4em (2)  $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$ or
\State \hskip4em (3) $m = ( JUSTIFICATION, \{m_x, m_y\} )$ with $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ and $x \neq y$:
\State \hskip6em \textbf{return} true

\State \hskip2em \textbf{else}
\State \hskip4em \textbf{return} false



\end{algorithmic}
\end{algorithm}

\begin{algorithm} 
\caption{\namebis: Pseudocode for process $P_i$}
\label{algorithm:wrapper-for-strong-validity}
\begin{algorithmic} [1]
\State \texttt{start} GroundWork
\State \textbf{upon} \texttt{terminate\_GroundWork}: \State \hskip2em \texttt{start} \name where a proposal $w$ is ignored in the PREPARE phase of any view iff no message $m$ s. t. $\texttt{legitimate}(m, w)$ has been delivered 
\end{algorithmic}
\end{algorithm}

\subsubsection{Proof of correctness of \namebis}

Here we prove the correctness of the algorithm \namebis.

\begin{lemma}[Validity]\label{lemma:sv-validity}
If all correct processes proposes the same value $w$, then
\begin{enumerate}
    \item every correct process receives (immediately from itself) a message $m = [ECHO, \sigma]$ with $Verify([PROPOSAL, w], \sigma)$
    \item No correct process delivers $M$ s. t. $\texttt{legitimate}(M, x)$ with $x \neq w$
\end{enumerate}
 
\end{lemma}

\begin{proof}
They are at least $2f+1$ broadcast of  messages of the form $[PROPOSAL, w]_{\sigma_j}$ (line \ref{line-gw:bcast-proposal}). Hence, every correct process receives $f+1$ messages of the form $[PROPOSAL, w]_{\sigma_j}$ (line \ref{line-gw:same-proposals}) and hence sends  $ [ECHO, \sigma]$ with $Verify([PROPOSAL, w], \sigma)$ (line \ref{line-gw:certify-same-proposals} and \ref{line-gw:bcast-echo}). This implies the item (1) of the lemma.
Moreover, the $f$ remaining processes cannot neither compute $ [ECHO, \sigma']$ with $Verify([PROPOSAL, x], \sigma')$ with $x \neq w$ nor compute $[JUSTIFICATION, \sigma_{\bot}]$ with $Verify([ECHO, \bot], \sigma_{\bot})$, since the threshold-scheme requires at least $f+1$ different share-signatures. 



\end{proof}

\begin{lemma}[Uniformity]\label{lemma:sv-uniformity}
If a correct process delivers $m$ by time $t$ s. t. $\texttt{legitimate}(m, w)$, then every correct process eventually receives $m'$ s. t. $\texttt{legitimate}(m', w)$ by time $max(GST, t) + \delta$.
\end{lemma}

\begin{proof}
Let $p$ be a correct process that terminates the GroundWork.
Necessarily, $p$ enter either in line \ref{line-gw:uniform-claim-not-same-proposals} or \ref{line-gw:at-least-two-different proposals} or in line \ref{line-gw:all-processes-consider-value-legitimate}. In first case, $p$ broadcast a JUSTIFICATION message (lines \ref{line-gw:certify-uniform-claim-not-same-proposals}and  \ref{line-gw:bcast-justification} or lines \ref{line-gw:certify-at-least-two-different-proposals} and  \ref{line-gw:bcast-justification-2} ) that legitimates all possible values. 
By justification's forwarding  (line \ref{line-gw:forward-justification}), if a justification message is received by a correct process by time $t$, then a justification message is received by each correct process by time $max(GST, t) + \delta$.
The only way to avoid that every correct process obtain a justification message before $GST + \delta$ is if all correct processes enter in line \ref{line-gw:all-processes-consider-value-legitimate}. But it is impossible that two correct processes enter in line \ref{line-gw:all-processes-consider-value-legitimate} for two different values. Hence they enter in line \ref{line-gw:all-processes-consider-value-legitimate} for one unique value $w$, which means they all received a message $m = [ECHO, \sigma_w]$ with $Verify([PROPOSAL, w], \sigma_w)$, which ends the proof.
\end{proof}



\begin{lemma}[Obligation]\label{lemma:sv-obligation}
After GST, for every correct leader $p$, its proposal is not ignored.  
\end{lemma}

\begin{proof}
Case 1: the proposal is its own proposal in \name.

This proposal has been chosen according to received messages in the groundWork algorithm.
$p$ entered either (i) in line \ref{line-gw:uniform-claim-not-same-proposals} or \ref{line-gw:at-least-two-different proposals} or (ii) in line \ref{line-gw:all-processes-consider-value-legitimate}.
In case (i), a JUSTIFICATION message will be received by every correct process by time $GST + \delta$.
In case (ii), the proposal has been updated to the relevant value so that every correct process receives $(ECHO, \sigma_w)$ with $Verify([PROPOSAL, w], \sigma_w)$.

Case 2: its proposal comes from the delivered $2f+1$ VIEW-CHANGE messages.

A VIEW-CHANGE message, encapsulates necessarily a value considered legitimate by at least $f+1$ correct processes by the quorum certificate.  The lemma holds by lemma \ref{lemma:sv-uniformity}.  
\end{proof}

\begin{lemma}[$O(n^2)$ complexity]\label{lemma:sv-complexity}
The communication complexity of the GroundWork algorithm is $O(n^2)$
\end{lemma}

\begin{proof}
Every correct process broadcast only one PROPOSAL message, one ECHO message and at most one JUSTIFICATION message where each message contains no more than ine threshold-signature and no more than share-signature.
\end{proof}

\begin{theorem}[Strong Validity]
 \namebis solves consensus with strong validity with $O(n^2)$ communication complexity. 
\end{theorem}

\begin{proof}
 The strong validity is ensured by lemma \ref{lemma:sv-validity}. The liveness of the algorithm is preserved by lemma \ref{lemma:sv-obligation}. The quadratic complexity is ensured by \ref{lemma:sv-complexity}
\end{proof}



\subsection{Drawbacks}

By synchronizing at each epoch only, the protocol suffers from some drawbacks that are discussed here.

\subsubsection{Clock Drift Tolerance}

Our model supposes that after GST, there is no clock drift, i.e. the real time is available to correct processes. It is legitimate to ask what happen if this assumption does not hold.
Let us investigate a less accomodating model where after GST, there exists a known bound $c > 1$ on clock drift. Without loss of generality, we assume that every correct process measures real time with a clock drift in $[1,c]$. Hence, if a correct process sets its timer to $c \cdot s$ seconds, when its timer expires, $s' \in [s, c \cdot s]$ real time seconds have elapsed.
The algorithm is slightly modified as follows: line 3 of algorithm 3 becomes $round\_timer$.measure$(k_{r} \cdot round\_duration$) where $k_{r}$ is an accurate coefficient, depending on round $r$ and clock drift bound $c$, to maintain the necessary and sufficient overlap of $8 \cdot \delta$ seconds at each round after first epoch synchronization after GST. In our case, setting $\forall r \in [1,f+1], k_{r} = c^{r}$ is necessary and sufficient to maintain the overlap (we fix $k_{0} = 0$). Indeed, for any $r \in [0,f+1]$, after $\tau_{r} = 2\delta + 10 \delta \cdot \sum_{i \in [1,r]} k_{i}$ real time seconds, the slowest process can enter in round $r+1$, while for any $r' \in [0,f]$, after $\tau'_{r'} = 10 \delta \cdot \sum_{i \in [1,r']} \frac{k_{i}}{c}$ real time seconds, the faster correct process can enter in round $r'+1$. To maintain the overlap, we want $\forall r \in [0,f]$, $\tau'_{r+1}- \tau_{r} \geq 8 \delta$. This lead us to $\forall r \in [0,f]$, $k_{r+1} \geq c +  (c-1) \cdot \sum_{i \in [1,r]} k_i $ and finally $\forall r \in [1,f+1]$, $k_{r} \geq c^{r}$ after an immediate induction. Thus, if we want to tolerate clock drift after GST, synchronizing at each epoch only leads to a worst-case latency complexity of $O(10 \delta \cdot c^{f})$, while synchronizing at each round, like in \cite{NBMS19, NK20}, leads to a worst-case latency complexity of $O(10 \delta \cdot c)$.

\subsubsection{Adaptiveness a.k.a. early stopping}

It is valuable to obtain complexity which depends on the \emph{actual} number $t$ of Byzantine processes instead of a bound $f$ on this number $t$. This property called adaptiveness or early-stopping is not ensured by our protocol. Indeed, we can imagine a scenario $S$ where at GST, the correct processes are partitioned in 3 groups of $f$ processes that are respectively in round $1$, $2$ and $3$ of the same epoch $e_{max}$. Then they will perform $O(f)$ rounds of epoch $e_{max}$ before triggering the round synchronization of epoch $e_{max + 1}$ and eventually agree on a common value, leading to a worst-case latency complexity of $O(\delta \cdot f)$ (and a worst-case communication complexity of $O(f \cdot n)$) . In the same scenario $S$, a protocol that synchronize at each round, like in \cite{NBMS19, NK20}, will perform $O(t)$ rounds before agreeing on a common value , leading to a worst-case latency complexity of $O(\delta \cdot t)$ (and a worst-case communication complexity of $O(t^2 \cdot n)$) .

\subsubsection{expected complexity}

Our protocol is designed to optimize worst-case complexity only, but neglect expected complexity, where the adversary does not choose the Byzantine processes according to the order of leaders. Again, because of scenario $S$, the expected complexity is the same than the worst-case complexity, that is an expected latency complexity of $O(\delta \cdot f)$ and an expected communication complexity of $O(f \cdot n)$. In the same scenario, protocol from $\cite{NK20}$ synchronize a $O(1)$ expected number of times, with a $O(n)$ expected communication complexity per round synchronization, leading to a $O(\delta)$ expected latency complexity and a $O(n)$ expected communication complexity. 

\begin{table}[]
\begin{tabular}{|l|ll|ll|ll|}
\hline
Protocols  & \multicolumn{2}{l|}{Complexity with clock drift}                                                                                                                & \multicolumn{2}{l|}{Adaptative Complexity}                                                         & \multicolumn{2}{l|}{Expected Complexity}                                                           \\ \hline
           & \multicolumn{1}{l|}{Latency}                                                                                   & Communication                                  & \multicolumn{1}{l|}{Latency}                                         & Communication               & \multicolumn{1}{l|}{Latency}                                         & Communication               \\ \hline
This paper & \multicolumn{1}{l|}{$O(\delta \cdot f \cdot c^f)$} & $O(f \cdot n)$                    & \multicolumn{1}{l|}{$O(\delta \cdot f)$} & $O(f \cdot n)$ & \multicolumn{1}{l|}{$O(\delta \cdot f)$} & $O(f \cdot n)$ \\ \hline
\cite{NK20}       & \multicolumn{1}{l|}{$O(\delta \cdot f \cdot c)$}                    & $O(f^2 \cdot n)$ & \multicolumn{1}{l|}{$O(\delta \cdot t)$} & $O(t \cdot n)$ & \multicolumn{1}{l|}{$O(\delta)$}                        & $O(n)$                        \\ \hline
\end{tabular}
\caption{Comparison between our solution and state-of-art solution \cite{NK20}. The only improvement is for worst-case communication complexity where we reach the Dolev-Reischuk bound}. We also meet the optimal worst-case latency complexity when there is no clock drift after GST.
\end{table}

\subsection{The naive view increasing synchronizer}


For sake of completeness, we rewrite (in slightly more general manner)  the analysis of (naive) view doubling synchronizer \cite{NBMS19} that enables quadratic communication complexity but with costly latency complexity exponential with the number of faulty processes.

In this approach, each view has a timer, and if no progress is made the node moves to the next view and increases the timer time for the next view, where we note $\beta$ the arbitrary duration of the first view. The view duration has to increase indefinitely not only for being able to exceed the unknown $c \cdot \delta$ overlap time, but also for enable late processes, that were the last ones to start the protocol, to catch up the most in advance ones, without synchronization.

The duration of view $v$ is so $\beta 2^{v-1}$.


\begin{algorithm} 
\caption{View doubling synchronizer: Pseudocode for process $P_i$}
\label{algorithm:view-doubling-synchronizer}
\begin{algorithmic} [1]


\State \textbf{initialize} : 
\State \hskip2em $current\_view \gets 1$
\State \hskip2em $view\_duration \gets \beta$ \Comment{$\beta$ is predefined value for the duration of the first view}

\State \textbf{upon} timer expiration: 
\State \hskip2em $view\_duration \gets 2\cdot view\_duration$ 
\State \hskip2em $start(current\_view +1)$

\end{algorithmic}
\end{algorithm}

\paragraph{Latency complexity with known $\delta$ standing after unknown $GST$}

\paragraph{Latency complexity with unknown $\delta$, unknown $GST$}

Let $E_{max}$ be the the maximum epoch where a correct process is when the last correct process start the protocol. 
Let us compute the view $v_d$ of decision in worst case. This view appears $O(f)$ views after $v_o$ which is the first view where correct processes overlap for time $d = constant \cdot \delta$.







==> sections/drawbacks.tex <==
\section{Drawbacks}\label{section:drawbacks}

By synchronizing at each epoch only, the protocol suffers from some drawbacks that are discussed here.



\subsection{Adaptiveness a.k.a. early stopping} \label{subsection:adaptiveness}

It is valuable to obtain complexity which depends on the \emph{actual} number $b$ of Byzantine processes instead of a bound $f$ on this number $b$. This property called adaptiveness (or early-stopping for the latency) is not ensured by our protocol. Indeed, we can imagine a scenario $S$ where at GST, the correct processes are partitioned in 3 groups of $f$ processes that are respectively in view $1$, $2$ and $3$ of the same epoch $e_{max}$. Then they will perform $O(f)$ views of epoch $e_{max}$ before triggering the view synchronization of epoch $e_{max + 1}$ and eventually agree on a common value, leading to a worst-case latency complexity of $O( f)$ (and a worst-case communication complexity of $O(f \cdot n)$) . In the same scenario $S$, a protocol that synchronize at each view, like in \cite{ Naor2020}, will perform $O(b)$ views before agreeing on a common value , leading to a worst-case latency complexity of $O(
b)$ (and a worst-case communication complexity of $O(b^2 \cdot n)$) .

\subsubsection{expected complexity}\label{subsection:expected_complexity}

Our protocol is designed to optimize worst-case complexity only, but neglects expected complexity, where the adversary does not choose the Byzantine processes according to the order of leaders. Again, because of scenario $S$, the expected complexity is the same than the worst-case complexity, that is an expected latency complexity of $O(f)$ and an expected communication complexity of $O(f \cdot n)$. In the same scenario, protocol from $\cite{Naor2020}$ synchronize a $O(1)$ expected number of times, with a $O(n)$ expected communication complexity per view synchronization, leading to a $O(1)$ expected latency complexity and a $O(n)$ expected communication complexity. 

\subsection{Clock Drift Tolerance}\label{subsection:clock_drift_tolerance}

Our model supposes that after GST, there is no clock drift, i.e. the real time is available to correct processes. It is legitimate to ask what happen if this assumption does not hold. 
Let us investigate a less accomodating model where after GST, there exists a known bound $c > 1$ on clock drift. Without loss of generality, we assume that every correct process measures real time with a clock drift in $[1,c]$. Hence, if a correct process sets its timer to $c \cdot s$ seconds, when its timer expires, $s' \in [s, c \cdot s]$ real time seconds have elapsed.
The algorithm \ref{algorithm:synchronizer} is slightly modified as follows: line \ref{line:view_timer_measure_without_msg_exchange} of algorithm \ref{algorithm:synchronizer}  becomes $view\_timer_i$.measure$(k_{v} \cdot view\_duration$) where $k_{v}$ is an accurate coefficient, depending on view $v$ and clock drift bound $c$, to maintain the necessary and sufficient overlap of $\Delta$ time at each view after first epoch synchronization after GST. In our case, setting $\forall v \in [1,f+1], k_{v} = c^{v}$ is necessary and sufficient to maintain the overlap (we fix $k_{0} = 0$). Indeed, for any $v \in [0,f+1]$, after $\tau_{v} = 2\delta + 10 \delta \cdot \sum_{i \in [1,v]} k_{i}$ real time, the slowest process can enter in view $v+1$, while for any $v' \in [0,f]$, after $\tau'_{v'} = 10 \delta \cdot \sum_{i \in [1,v']} \frac{k_{i}}{c}$ real time, the faster correct process can enter in view $v'+1$. To maintain the overlap, we want $\forall v \in [0,f]$, $\tau'_{v+1}- \tau_{v} \geq \Delta$. This lead us to $\forall v \in [0,f]$, $k_{v+1} \geq c +  (c-1) \cdot \sum_{i \in [1,v]} k_i $ and finally $\forall r \in [1,f+1]$, $k_{v} \geq c^{v}$ after an immediate induction. Thus, if we want to tolerate clock drift after GST, synchronizing at each epoch only leads to a worst-case latency complexity of $O(10 \delta \cdot c^{f})$, while synchronizing at each view, like in \cite{Naor2020}, leads to a worst-case latency complexity of $O(10 \delta \cdot c)$.

\begin{table}[]
\begin{tabular}{|l|ll|ll|ll|}
\hline
Protocols  & \multicolumn{2}{l|}{Complexity with clock drift}                                                                                                                & \multicolumn{2}{l|}{Adaptative Complexity}                                                         & \multicolumn{2}{l|}{Expected Complexity}                                                           \\ \hline
           & \multicolumn{1}{l|}{Latency}                                                                                   & Communication                                  & \multicolumn{1}{l|}{Latency}                                         & Communication               & \multicolumn{1}{l|}{Latency}                                         & Communication               \\ \hline
This paper & \multicolumn{1}{l|}{$O( f \cdot c^f)$} & $O(f \cdot n)$                    & \multicolumn{1}{l|}{$O(f)$} & $O(f \cdot n)$ & \multicolumn{1}{l|}{$O(f)$} & $O(f \cdot n)$ \\ \hline
\cite{Naor2020}       & \multicolumn{1}{l|}{$O(b \cdot c)$}                    & $O(b^2 \cdot n)$ & \multicolumn{1}{l|}{$O(b)$} & $O(b^2 \cdot n)$ & \multicolumn{1}{l|}{$O(1)$}                        & $O(n)$                        \\ \hline
\end{tabular}
\caption{Comparison between our solution and state-of-art solution \cite{Naor2020}. The only improvement is for worst-case communication complexity where we reach the Dolev-Reischuk bound}. We also meet the optimal worst-case latency complexity when there is no clock drift after GST.
\end{table}




==> sections/generalized_lower_bound.tex <==
\section{Generalized Dolev-Reischuk Bound}

Dolev-Reischuk lower bound~\cite{dolev1985bounds} claims that any Byzantine consensus protocol operating in a partially synchronous environment has $\Omega(f^2)$ communication complexity, where $f$ represents the number of tolerated Byzantine processes.
However, Dolev and Reischuk consider the Byzantine consensus problem satisfying \emph{strong validity:} if all correct processes propose the same value $v$, then only value $v$ can be decided by a correct process.
The question is whether the quadratic lower bound holds for Byzantine consensus problems satisfying some other variant of the validity property.
In this section, we define an attribute $\mathcal{A}$, which is defined as a set of executions, such that, if a partially synchronous Byzantine consensus protocol satisfies $\mathcal{A}$, then the Dolev-Reischuk lower bound applies to the protocol.

We fix $\Pi$, a Byzantine consensus protocol operating in a partially synchronous model (either $\mathcal{PS}_{\delta}$ or $\mathcal{PS}_{\mathit{GST}, \delta}$) among $n$ processes out of which  $0 < f < n$ can be faulty.
Protocol $\Pi$ satisfies the following properties:
\begin{compactitem}
    \item \emph{Termination:} All correct processes eventually decide.
    
    \item \emph{Agreement:} All correct processes decide the same value. \pierre{If we want to write agreement property as a safety property (that is not redundant with termination), we should write "no pair of correct processes disagree }
    
    \item \emph{Validity:} Some validity property. \pierre{(1)You meant some additional safety property ? } %\pierre{(2) Later, it seems to me that "very weak validity" is assumed, i. e. if all processes are correct and propose the same value $v \in \mathbb{V}$, then $v$ is the only value that can be decided, which seems weaker than $\mathcal{A}$, but I need to check first}
    
    %\pierre{(2) Another "hyper weak validity" could, i. e. if all processes are correct and propose the same value $v \in \mathbb{V}$, then $v$ is the only value that can be decided, which seems weaker than $\mathcal{A}$, but I need to check first}
\end{compactitem}
Let $\mathbb{V}$ denote the set of all values that can be proposed (and decided) in executions of $\Pi$.

Let us fix two disjoint groups of processes executing $\Pi$: (1) group $U$, where $|U| = n - \lceil f / 2 \rceil$, and (2) group $V$, where $|V| = \lceil f / 2 \rceil$.
For every value $v \in \mathbb{V}$, we define the set of executions $\mathit{execs}_{\Pi}(U, V, v)$ such that $e \in \mathit{execs}_{\Pi}(U, V, v)$ if and only if the following holds for $e$:
\begin{compactitem}
    \item All processes in the $U$ group are correct in $e$, whereas all processes in the $V$ group are faulty in $e$.
    
    \item No process in the $V$ group sends any message in $e$, i.e., these processes are silent in $e$.
    
    \item All processes in the $U$ group propose $v \in \mathbb{V}$ in $e$.
\end{compactitem}

We are ready to define when $\Pi$ satisfies attribute $\mathcal{A}$.

\begin{definition} [Satisfaction of attribute $\mathcal{A}$]
Protocol $\Pi$ \emph{satisfies attribute $\mathcal{A}$} if and only if there exist disjoint groups $U$ and $V$, where $|U| = n - \lceil f / 2 \rceil$ and $|V| = \lceil f / 2 \rceil$, such that, for every value $v \in \mathbb{V}$ \pierre{I guess "for every value $v \in \mathbb{V}$" can be replaced by "for two different values $v, v' \in \mathbb{V}$" s. t. the result still holds with an even weaker attribute} and every execution $e \in \mathit{execs}_{\Pi}(U, V, v)$, all correct processes decide $v$ in $e$.
\end{definition}

Intuitively, $\Pi$ satisfies $\mathcal{A}$ if and only if all correct processes decide the common proposed value in \emph{all} executions in which they propose the same value and faulty processes are silent.
Next, we prove that $\Pi$, a Byzantine consensus protocol satisfying $\mathcal{A}$, has $\Omega(f^2)$ communication complexity.

\begin{theorem} \label{theorem:generalized_dolev}
Let $\Pi$ be any Byzantine consensus protocol operating in a partially synchronous environment~\cite{dwork1988consensus} among $n$ processes out of which $0 < f < n$ can be faulty and let $\Pi$ satisfy $\mathcal{A}$.
The communication complexity of $\Pi$ is $\Omega(f^2)$.
\pierre{In fact we can say consensus protocol (non Byzantine) and $f$ processes can perform omission faults.} \jovan{Yes. But, I probably would not introduce that. It might introduce some confusion that is unnecessary. I would stick to Byzantine. What do you think?} \pierre{You are right. Perhaps at the end of the demonstration, we can mention that the "attack" from $U_i$ and $V$ used only omission faults.}
\end{theorem}
\begin{proof}
We fix a value $v \in \mathbb{V}$.
Let $e \in \mathit{execs}_{\Pi}(U, V, v)$ be an execution in which all correct processes (i.e., the processes in the $U$ group) propose and decide $v$.
By contradiction, suppose that correct processes send less than $(\lfloor f / 2 \rfloor)^2$ messages in $e$ (otherwise, the communication complexity of $\Pi$ would be $\Omega(f^2)$).
By the pigeonhole principle, there exists a process $P_i \in V$ that receives less than $\lfloor f / 2 \rfloor$ messages in $e$.
We denote by $U_i \subset U$ the set of correct processes that send messages to $P_i$ in $e$; note that $|U_i| \leq \lfloor f / 2 \rfloor$.

Now, we construct an execution $e'$ of $\Pi$:
\begin{compactitem}
    \item All processes in the $U \setminus{U_i}$ set are correct.
    Moreover, process $P_i$ is correct.
    
    \item Processes in the $V \setminus{\{P_i\}}$ set are faulty and silent, i.e., they do not send any message. 
    
    \item Processes in the $U_i$ set are faulty and behave exactly as they do in $e$, except that they do not send any message to $P_i$.
    
    \item Execution $e'$ is indistinguishable from $e$ to processes in the $U \setminus{U_i}$ set.
\end{compactitem}
Note that $e'$ has (at most) $f - 1$ faulty processes ($\lceil f / 2 \rceil - 1$ faults in the group $V$ and $\lfloor f / 2 \rfloor $ faults in the group $U$).
Moreover, all processes in the $U \setminus{U_i}$ set decide $v$ (since they do not distinguish $e'$ from $e$ until their decision).
Finally, $P_i$ does not receive any message in $e'$; moreover, $P_i$ decides $v$ in $e'$ (because of the termination and agreement properties satisfied by $\Pi$).

Lastly, we create an execution $e''$ in the following manner:
\begin{compactenum}
    \item We take an execution $e_{v'} \in \mathit{execs}_{\Pi}(U, V, v')$, where $v' \neq v$.
    
    \item We make process $P_i \in V$ correct.
    
    \item Messages sent by process $P_i$ are not received before processes in the group $U$ decide $v'$ (since $e''$ is indistinguishable from $e_{v'}$ to them).
    
    \item Messages sent to process $P_i$ are delayed until $P_i$ decides $v$ (since $e''$ is indistinguishable from $e'$ to $P_i$).
\end{compactenum}
Therefore, the agreement property is violated in $e''$.
We reach a contradiction with the fact that $\Pi$ solves the Byzantine consensus protocol, which concludes the proof of the theorem.
\end{proof}

We conclude the section by listing some noteworthy versions of the validity property which ensure that any Byzantine consensus protocol guaranteeing them satisfies attribute $\mathcal{A}$:
\begin{compactitem}
    \item Weak validity: If all processes are correct, then the value decided by a correct process was proposed by a correct process.
    
    \emph{Why is $\mathcal{A}$ satisfied?}
    Let $\Pi$ be any Byzantine consensus protocol guaranteeing weak validity.
    We fix any two disjoint groups $U$ and $V$, where $|U| = n - \lceil f / 2 \rceil$ and $|V| = \lceil f / 2 \rceil$.
    For every value $v \in \mathbb{V}$ and every execution $e \in \mathit{execs}_{\Pi}(U, V, v)$, processes in the group $U$ must decide $v$; otherwise, there exists an execution in which (1) all processes are correct and all processes propose $v$, (2) messages from the group $V$ to the group $U$ are delayed, and (3) correct processes in the group $U$ decide a value different than $v$, which violates weak validity.
    
    \item Strong validity (variant 1): If all correct processes propose the same value $v$, then only value $v$ can be decided by a correct process.
    
    \emph{Why is $\mathcal{A}$ satisfied?} \pierre{Perhaps we can say that strong validity implies weak validity ?}
    Let $\Pi$ be any Byzantine consensus protocol guaranteeing this version of validity.
    We fix any two disjoint groups $U$ and $V$, where $|U| = n - \lceil f / 2 \rceil$ and $|V| = \lceil f / 2 \rceil$.
    For every value $v \in \mathbb{V}$ and every execution $e \in \mathit{execs}_{\Pi}(U, V, v)$, processes in the group $U$ must decide $v$ since all correct processes have proposed $v$.
    
    \item Strong validity (variant 2): If a correct process decides a value $v$, then $v$ was proposed by a correct process.
    
    \emph{Why is $\mathcal{A}$ satisfied?} \pierre{Perhaps we can say that strong validity implies weak validity ?}
    Let $\Pi$ be any Byzantine consensus protocol guaranteeing this version of validity.
    We fix any two disjoint groups $U$ and $V$, where $|U| = n - \lceil f / 2 \rceil$ and $|V| = \lceil f / 2 \rceil$.
    For every value $v \in \mathbb{V}$ and every execution $e \in \mathit{execs}_{\Pi}(U, V, v)$, processes in the group $U$ must decide $v$ since correct processes have proposed only $v$.
    
    \item External validity: Let the domain of the valid values be unknown.
    At the beginning of every execution, each correct process gets a value $v$ to propose accompanied with a proof $\sigma$ that $v$ is valid.
    Moreover, it is computationally impossible for a correct process to create a proof $\sigma'$ that some value $v'$ is valid, where $v'$ is not the proposed value of the process.
    Finally, if a correct process decides a value, then the value is accompanied by a proof that the value is valid.\footnote{External validity captures the validity property traditionally incorporated in blockchains in which each process proposes a block of (properly signed) transactions issued by clients.}
    
    \emph{Why is $\mathcal{A}$ satisfied?}
    Let $\Pi$ be any Byzantine consensus protocol guaranteeing external validity.
    We fix any two disjoint groups $U$ and $V$, where $|U| = n - \lceil f / 2 \rceil$ and $|V| = \lceil f / 2 \rceil$.
    For every value $v \in \mathbb{V}$ and every execution $e \in \mathit{execs}_{\Pi}(U, V, v)$, processes in the group $U$ must decide $v$ since correct processes do not ``discover'' any other valid value.
    Recall that a correct process is incapable of producing a proof for a non-proposed value and that a correct process cannot verify that a value is valid unless it obtains a proof for the value.
\end{compactitem}
If a Byzantine consensus protocol guarantees any of the aforementioned versions of validity, the protocol has $\Omega(f^2)$ communication complexity (by \Cref{theorem:generalized_dolev}).
In the case of $f = O(n)$, the communication complexity is $\Omega(n^2)$.

==> sections/round_synchronization.tex <==
\section{\rare} \label{section:rare}

This section presents \rare, a partially synchronous view synchronizer that achieves synchronization within $O(f)$ time after $\mathit{GST}$, and has $O(n^2)$ worst-case communication complexity.
First, we define the problem of view synchronization (\Cref{subsection:view_synchronization_problem_definition}).
Then, we describe \rare, and present its pseudocode (\Cref{subsection:rare}).
Finally, we reason about \rare's correctness and complexity (\Cref{subsection:rare_proof_sketch}).
% Finally, we discuss \rare's drawbacks in \Cref{subsection:drawbacks}. 

% The formal proof of \rare's correctness and complexity is delegated to \Cref{section:appendix_rare}.

\subsection{Problem Definition} \label{subsection:view_synchronization_problem_definition}

View synchronization is defined as the problem of bringing all correct processes to the same view with a correct leader for sufficiently long~\cite{Bravo2020,Naor2020, Naor2021}.
More precisely, let $\mathsf{View} = \{1, 2, ...\}$ denote the set of views.
For each view $v \in \mathsf{View}$, we define $\mathsf{leader}(v)$ to be a process that is the \emph{leader} of view $v$.
The view synchronization problem is associated with a predefined time $\Delta > 0$, which denotes the desired duration during which processes must be in the same view with a correct leader in order to synchronize.
View synchronization provides the following interface:
\begin{compactitem}
    \item \textbf{Indication} $\mathsf{advance}(\mathsf{View} \text{ } v)$: The process advances to a view $v$.
\end{compactitem}
We say that a correct process \emph{enters} a view $v$ at time $t$ if and only if the $\mathsf{advance}(v)$ indication occurs at time $t$.
Moreover, a correct process \emph{is in view} $v$ between the time $t$ (including $t$) at which the $\mathsf{advance}(v)$ indication occurs and the time $t'$ (excluding $t'$) at which the next $\mathsf{advance}(v' \neq v)$ indication occurs.
If an $\mathsf{advance}(v' \neq v)$ indication never occurs, the process remains in the view $v$ from time $t$ onward.

Next, we define a \emph{synchronization time} as a time at which all correct processes are in the same view with a correct leader for (at least) $\Delta$ time.

\begin{definition} [Synchronization time] \label{definition:synchronization_time}
Time $t_s$ is a \emph{synchronization time} if (1) all correct processes are in the same view $v$ from time $t_s$ to (at least) time $t_s + \Delta$, and (2) $\mathsf{leader}(v)$ is correct.
\end{definition}

View synchronization ensures the \emph{eventual synchronization} property which states that there exists a synchronization time at or after $\mathit{GST}$.

\smallskip
\noindent \textbf{Complexity of view synchronization.}
Let $\mathsf{Synchronizer}$ be a partially synchronous view synchronizer and let $\mathcal{E}(\mathsf{Synchronizer})$ denote the set of all possible executions.
Let $\alpha \in \mathcal{E}(\mathsf{Synchronizer})$ be an execution and $t_s(\alpha)$ be the first synchronization time at or after $\mathit{GST}$ in $\alpha$ ($t_s(\alpha) \geq \mathit{GST}$).
We define the communication complexity of $\alpha$ as the number of words sent in messages by all correct processes during the time period $[\mathit{GST}, t_s(\alpha) + \Delta]$.
The latency complexity of $\alpha$ is $t_s(\alpha) + \Delta - \mathit{GST}$.

The \emph{communication complexity} of $\mathsf{Synchronizer}$ is defined as
\begin{equation*}
\max_{\alpha \in \mathcal{E}(\mathsf{Synchronizer})}\bigg\{\text{communication complexity of } \alpha\bigg\}.
\end{equation*}

Similarly, the \emph{latency complexity} of $\mathsf{Synchronizer}$ is defined as 
\begin{equation*}
\max_{\alpha \in \mathcal{E}(\mathsf{Synchronizer})}\bigg\{\text{latency complexity of } \alpha\bigg\}.
\end{equation*}

\iffalse
\subsection{Naive Implementation}

We rewrite the analysis of naive view doubling synchronizer (already presented in \cite{NBMS20}) that enables quadratic communication complexity but with costly latency complexity exponential with the number of faulty processes.

In this approach, each view has a timer, and if no progress is made the node moves to the next view and increases the timer time for the next view, where we note $\beta$ the arbitrary duration of the first view. The view duration has to increase indefinitely to enable late processes, (e.g. last ones that started the protocol or the ones with the slowest clocks), to catch up the most in advance ones, without communication.
To do this, the duration of a view $v$ has to be greater than the duration of the sum of all previous views up to view $v-1$, which lead us to an exponential pattern. Typically the duration of view $v$ is $\beta \cdot 2^{v-1}$ (The constant $2$ can be replaced by any value strictly greater than $1$).


\begin{algorithm} 
\caption{View doubling synchronizer: Pseudocode for process $P_i$}
\label{algorithm:view-doubling-synchronizer}
\begin{algorithmic} [1]


\State \textbf{initialize} : 
\State \hskip2em $current\_view \gets 1$
\State \hskip2em $view\_duration \gets \beta$ \BlueComment{$\beta$ is predefined value for the duration of the first view}

\State \textbf{upon} timer expiration: 
\State \hskip2em $view\_duration \gets 2\cdot view\_duration$ 
\State \hskip2em $start(current\_view +1)$

\end{algorithmic}
\end{algorithm}

This synchronizer possesses the advantage of a free communication, but suffer from an unbounded latency complexity. Indeed, even without clock drift, if the most in advance correct process start the protocol at time $0$, while the most late correct process start the protocol at time $GST$.



%it is possible for a correct process to enter in first view, while another 
Indeed, at GST, a correct process can enter in the first view, while
there is no bound on the view $v_{max}$ of the most in advance process. Hence, the synchronization time will not be met before time $\beta\cdot 2^{v_{max}}$ which is unbounded.
\fi

\subsection{Protocol} \label{subsection:rare}

This subsection details \rare (\Cref{algorithm:synchronizer}).
% We now detail \rare (\Cref{algorithm:synchronizer})
% , a view synchronizer with $O(n^2)$ communication complexity and $O(f)$ latency complexity.
In essence, \rare achieves $O(n^2)$ communication complexity and $O(f)$ latency complexity by exploiting ``all-to-all'' communication only once per $f + 1$ views.

\smallskip 
\noindent \textbf{Intuition.}
We group views into \emph{epochs}, where each epoch contains $f + 1$ sequential views; $\mathsf{Epoch} = \{1, 2, ...\}$ denotes the set of epochs.
Processes move through an epoch solely by means of local timeouts (without any communication).
However, at the end of each epoch, processes engage in an ``all-to-all'' communication step to obtain permission to move onto the next epoch: (1) Once a correct process has completed an epoch, it broadcasts a message informing other processes of its completion; (2) Upon receiving $2f + 1$ of such messages, a correct process enters the future epoch. Note that (2) applies to \emph{all} processes, including those in arbitrarily ``old'' epochs.
Overall, this ``all-to-all'' communication step is the \emph{only} communication processes perform within a single epoch, implying that per-process communication complexity in each epoch is $O(n)$.
\Cref{fig:raresync} illustrates the main idea behind \rare.


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.2]{figures/raresync.png}
    \caption{Intuition behind \rare: Processes communicate only in the last view of an epoch; before the last view, they rely solely on local timeouts.}
    \label{fig:raresync}
\end{figure}

Roughly speaking, after $\mathit{GST}$, all correct processes simultaneously enter the same epoch within $O(f)$ time.
After entering the same epoch, processes are guaranteed to synchronize in that epoch, which takes (at most) an additional $O(f)$ time.
Thus, the latency complexity of \rare is $O(f)$.
The communication complexity of \rare is $O(n^2)$ as every correct process executes at most a constant number of epochs, each with $O(n)$ per-process communication, after $\mathit{GST}$.


\smallskip
\noindent \textbf{Protocol description.}
We now explain how \rare works.
The pseudocode of \rare is given in \Cref{algorithm:synchronizer}, whereas all variables, constants, and functions are presented in \Cref{algorithm:variable_constants}.

\begin{algorithm} [b]
\caption{\rare: Variables (for process $P_i$), constants, and functions}
\label{algorithm:variable_constants}
\begin{algorithmic} [1]

\State \textbf{Variables:}
\State \hskip2em $\mathsf{Epoch}$ $\mathit{epoch}_i \gets 1$ \BlueComment{current epoch}
\State \hskip2em $\mathsf{View}$ $\mathit{view}_i \gets 1$ \BlueComment{current view within the current epoch; $\mathit{view}_i \in [1, f + 1]$}  \label{line:init_view}
\State \hskip2em $\mathsf{Timer}$ $\mathit{view\_timer}_i$ \BlueComment{measures the duration of the current view}
\State \hskip2em $\mathsf{Timer}$ $\mathit{dissemination\_timer}_i$ \BlueComment{measures the duration between two communication steps}
\State \hskip2em $\mathsf{T\_Signature}$ $\mathit{epoch\_sig}_i \gets \bot$ \BlueComment{proof that $\mathit{epoch}_i$ can be entered}

\smallskip
\State \textbf{Constants:}
\State \hskip2em $\mathsf{Time}$ $\mathit{view\_duration} = \Delta + 2\delta$ \BlueComment{duration of each view} \label{line:view_duration}

\smallskip
\State \textbf{Functions:}
\State \hskip2em $\mathsf{leader}(\mathsf{View} \text{ } v) \equiv P_{(v \text{ } \mathsf{mod} \text{ } n) + 1}$ \BlueComment{a round-robin function} \label{line:leader_rare}
\end{algorithmic}
\end{algorithm} 

\begin{algorithm} [t]
\caption{\rare: Pseudocode (for process $P_i$)}
\label{algorithm:synchronizer}
\begin{algorithmic} [1]


\State \textbf{upon} $\mathsf{init}$: \BlueComment{start of the protocol} \label{line:start_algorithm}

\State \hskip2em
$\mathit{view\_timer}_i.\mathsf{measure(}\mathit{view\_duration}\mathsf{)}$ \BlueComment{measure the duration of the first view} \label{line:view_timer_measure_first_view} 

\State \hskip2em \textbf{trigger} $\mathsf{advance(}1\mathsf{)}$ \label{line:start_view_1} \BlueComment{enter the first view}

\smallskip
\State \textbf{upon} $\mathit{view\_timer}_i$ \textbf{expires}:
\label{line:rule_view_expired}
\State \hskip2em \textbf{if} $\mathit{view}_i < f + 1$: \BlueComment{check if the current view is not the last view of the current epoch} \label{line:check_last_view}
\State \hskip4em $\mathit{view}_i \gets \mathit{view}_i + 1$ \label{line:increment_view}
\State \hskip4em $\mathsf{View}$ $\mathit{view\_to\_advance} \gets (\mathit{epoch}_i - 1) \cdot (f + 1) + \mathit{view}_i$

%%
\State \hskip4em
$\mathit{view\_timer}_i.\mathsf{measure(}\mathit{view\_duration}\mathsf{)}$ \BlueComment{measure the duration of the view} \label{line:view_timer_measure_without_msg_exchange} 

\State \hskip4em \textbf{trigger} $\mathsf{advance(}\mathit{view\_to\_advance}\mathsf{)}$ \label{line:start_view_without_msg_exchange} \BlueComment{enter the next view}
%%

%\State \hskip4em \textbf{trigger} \texttt{start\_view} \BlueComment{start the next view of the current epoch}
\State \hskip2em \textbf{else:}
\State \hskip4em \textcolor{blue}{\(\triangleright\) inform other processes that the epoch is completed}
\State \hskip4em \textbf{broadcast} $\langle \textsc{epoch-completed}, \mathit{epoch}_i, \mathit{ShareSign}_i(\mathit{epoch}_i) \rangle$ \label{line:broadcast_epoch_over}

\smallskip
\State \textbf{upon} exists $\mathsf{Epoch}$ $e$ such that $e \geq \mathit{epoch}_i$ and $\langle \textsc{epoch-completed}, e, \mathsf{P\_Signature} \text{ } \mathit{sig} \rangle$ is received from $2f + 1$ processes: \label{line:receive_epoch_over}
%\State \hskip2em \st{\textbf{trigger} \texttt{terminate\_view}} 
\State \hskip2em $\mathit{epoch\_sig}_i \gets \mathit{Combine}\big(\{\mathit{sig} \,|\, \mathit{sig} \text{ is received in an } \textsc{epoch-completed} \text{ message}\}\big)$ \label{line:combine-signatures}
\State \hskip2em $\mathit{epoch}_i \gets e + 1$  \label{line:update_epoch_1} %\BlueComment{enter $\mathit{epoch}$}
\State \hskip2em
$\mathit{view\_timer}_i.\mathsf{cancel()}$ \label{line:cancel_view_timer_1}
\State \hskip2em $\mathit{dissemination\_timer}_i.\mathsf{cancel()}$ \label{line:sync_timer_cancel_1}
\State \hskip2em $\mathit{dissemination\_timer}_i.\mathsf{measure(}\delta\mathsf{)}$ \label{line:sync_timer_measure} \BlueComment{wait $\delta$ time before broadcasting \textsc{enter-epoch}}

\smallskip
\State \textbf{upon} reception of $\langle \textsc{enter-epoch}, \mathsf{Epoch} \text{ } e, \mathsf{T\_Signature} \text{ } \mathit{sig} \rangle$ such that $e > \mathit{epoch}_i$: \label{line:receive_epoch_over_complete}
%\State \hskip2em \st{\textbf{trigger} \texttt{terminate\_view}} 
\State \hskip2em $\mathit{epoch\_sig}_i \gets \mathit{sig}$ \label{line:adopt_signature} \BlueComment{$\mathit{sig}$ is a threshold signature of epoch $e - 1$}
\State \hskip2em $\mathit{epoch}_i \gets e$  \label{line:update_epoch_2} %\BlueComment{enter $\mathit{epoch}$}
\State \hskip2em
$\mathit{view\_timer}_i.\mathsf{cancel()}$ \label{line:cancel_view_timer_2}
\State \hskip2em $\mathit{dissemination\_timer}_i.\mathsf{cancel()}$  \label{line:sync_timer_cancel_2}
\State \hskip2em $\mathit{dissemination\_timer}_i.\mathsf{measure(}\delta\mathsf{)}$ \label{line:sync_timer_measure_2} \BlueComment{wait $\delta$ time before broadcasting \textsc{enter-epoch}}

\smallskip
\State \textbf{upon} $\mathit{dissemination\_timer}_i$ \textbf{expires}: \label{line:sync_timer_expires}
\State \hskip2em \textbf{broadcast} $\langle \textsc{enter-epoch}, \mathit{epoch}_i, \mathit{epoch\_sig}_i \rangle$ \label{line:broadcast_epoch_over_complete}
\State \hskip2em $\mathit{view}_i \gets 1$ \BlueComment{reset the current view to $1$} \label{line:reset_view}
\State \hskip2em $\mathsf{View}$ $\mathit{view\_to\_advance} \gets (\mathit{epoch}_i - 1) \cdot (f + 1) + \mathit{view}_i$

\State \hskip2em
$\mathit{view\_timer}_i.\mathsf{measure(}\mathit{view\_duration}\mathsf{)}$   \label{line:view_timer_measure} \BlueComment{measure the duration of the view}

\State \hskip2em \textbf{trigger} $\mathsf{advance(}\mathit{view\_to\_advance}\mathsf{)}$ \label{line:start_view_2} \BlueComment{enter the first view of the new epoch}



\end{algorithmic}
\end{algorithm}

We explain \rare's pseudocode (\Cref{algorithm:synchronizer}) from the perspective of a correct process $P_i$.
Process $P_i$ utilizes two timers: $\mathit{view\_timer}_i$ and $\mathit{dissemination\_timer}_i$.
A timer has two methods:
\begin{compactenum}
    \item $\mathsf{measure}(\mathsf{Time} \text{ } x)$: After exactly $x$ time as measured by the local clock, an expiration event is received by the host.
    Note that, as local clocks can drift before $\mathit{GST}$, $x$ time as measured by the local clock may not amount to $x$ real time (before $\mathit{GST}$).
    \item $\mathsf{cancel()}$: 
    This method cancels all previously invoked $\mathsf{measure}(\cdot)$ methods on that timer, i.e., all pending expiration events (pertaining to that timer) are removed from the event queue.
\end{compactenum}
In \rare, $\mathsf{leader}(\cdot)$ is a round-robin function (line~\ref{line:leader_rare} of \Cref{algorithm:variable_constants}).

Once $P_i$ starts executing $\rare$ (line~\ref{line:start_algorithm}), it instructs $\mathit{view\_timer}_i$ to measure the duration of the first view (line~\ref{line:view_timer_measure_first_view}) and it enters the first view (line~\ref{line:start_view_1}).

Once $\mathit{view\_timer}_i$ expires (line~\ref{line:rule_view_expired}), $P_i$ checks whether the current view is the last view of the current epoch, $\mathit{epoch}_i$ (line~\ref{line:check_last_view}).
If that is not the case, the process advances to the next view of $\mathit{epoch}_i$ (line~\ref{line:start_view_without_msg_exchange}).
Otherwise, the process broadcasts an $\textsc{epoch-completed}$ message (line~\ref{line:broadcast_epoch_over}) signaling that it has completed $\mathit{epoch}_i$.
At this point in time, the process does not enter any view.

If, at any point in time, $P_i$ receives either (1) $2f + 1$ $\textsc{epoch-completed}$ messages for some epoch $e \geq \mathit{epoch}_i$ (line~\ref{line:receive_epoch_over}), or (2) an \textsc{enter-epoch} message for some epoch $e' > \mathit{epoch}_i$ (line~\ref{line:receive_epoch_over_complete}), the process obtains a proof that a new epoch $E > \mathit{epoch}_i$ can be entered.
However, before entering $E$ and propagating the information that $E$ can be entered, $P_i$ waits $\delta$ time (either line~\ref{line:sync_timer_measure} or line~\ref{line:sync_timer_measure_2}).
This $\delta$-waiting step is introduced to limit the number of epochs $P_i$ can enter within any $\delta$ time period after $\mathit{GST}$ and is crucial for keeping the communication complexity of \rare quadratic.
For example, suppose that processes are allowed to enter epochs and propagate \textsc{enter-epoch} messages without waiting.
Due to an accumulation (from before $\mathit{GST}$) of \textsc{enter-epoch} messages for different epochs, a process might end up disseminating an arbitrary number of these messages by receiving them all at (roughly) the same time.
To curb this behavior, given that message delays are bounded by $\delta$ after $\mathit{GST}$, we force a process to wait $\delta$ time, during which it receives all accumulated messages, before entering the largest known epoch.

Finally, after $\delta$ time has elapsed (line~\ref{line:sync_timer_expires}), $P_i$ disseminates the information that the epoch $E$ can be entered (line~\ref{line:broadcast_epoch_over_complete}) and it enters the first view of $E$ (line~\ref{line:start_view_2}).

\subsection{Correctness and Complexity: Proof Sketch} \label{subsection:rare_proof_sketch}

This subsection presents a proof sketch of the correctness, latency complexity, and communication complexity of \rare. The full proof can be found in \Cref{section:appendix_rare}.

In order to prove the correctness of \rare, we must show that the eventual synchronization property is ensured, i.e., there is a synchronization time $t_s \geq \mathit{GST}$.
For the latency complexity, it suffices to bound $t_s + \Delta - \mathit{GST}$ by $O(f)$.
This is done by proving that synchronization happens within (at most) 2 epochs after $\mathit{GST}$.
% , i.e., $(t_s + \Delta - \mathit{GST}) \leq 2 \cdot \textit{epoch\_duration} + 4\delta = O(f)$, where $\mathit{epoch\_duration} = (f + 1) \cdot \mathit{view\_duration}$. 
As for the communication complexity, we prove that any correct process enters a constant number of epochs during the time period $[\mathit{GST}, t_s + \Delta]$. 
Since every correct process sends $O(n)$ words per epoch, the communication complexity of \rare is $O(n^2) = O(1) \cdot O(n) \cdot n$. %\ayaz{minor, can ignore. I think it looks better if we reverse the equation, i.e $O(1) \cdot O(n) \cdot n = O(n^2)$}
We work towards these conclusions by introducing some key concepts and presenting a series of intermediate results.

A correct process \emph{enters} an epoch $e$ at time $t$ if and only if the process enters the first view of $e$ at time $t$ (either line~\ref{line:start_view_1} or line~\ref{line:start_view_2}).
We denote by $t_e$ the first time a correct process enters epoch $e$.

\smallskip
\noindent \textbf{Result 1:} \emph{If a correct process enters an epoch $e > 1$, then (at least) $f + 1$ correct processes have previously entered epoch $e - 1$.} % lock step
\smallskip
\\ The goal of the communication step at the end of each epoch is to prevent correct processes from arbitrarily entering future epochs. 
In order for a new epoch $e > 1$ to be entered, at least $f + 1$ correct processes must have entered and ``gone through'' each view of the previous epoch, $e - 1$. 
This is indeed the case: in order for a correct process to enter $e$, the process must either (1) collect $2f + 1$ $\textsc{epoch-completed}$ messages for $e - 1$ (line~\ref{line:receive_epoch_over}), or (2) receive an \textsc{enter-epoch} message for $e$, which contains a threshold signature of $e - 1$ (line~\ref{line:receive_epoch_over_complete}). 
In either case, at least $f + 1$ correct processes must have broadcast $\textsc{epoch-completed}$ messages for epoch $e - 1$ (line~\ref{line:broadcast_epoch_over}), which requires them to go through epoch $e - 1$.
Furthermore, $t_{e - 1} \leq t_{e}$; recall that local clocks can drift before $\mathit{GST}$.
% , for every epoch $e > 1$.
% (lines~\ref{line:rule_view_expired} to~\ref{line:start_view_without_msg_exchange}).

\smallskip
\noindent \textbf{Result 2:} \emph{Every epoch is eventually entered by a correct process.}
\smallskip
\\By contradiction, consider the greatest epoch ever entered by a correct process, $e^*$.
% Let $t_{e^*}$ denote the first time a correct process enters $e^*$.
In brief, every correct process will eventually (1) receive the \textsc{enter-epoch} message for $e^*$ (line~\ref{line:receive_epoch_over_complete}), (2) enter $e^*$ after its $\mathit{dissemination\_timer}$ expires (lines~\ref{line:sync_timer_expires} and~\ref{line:start_view_2}), (3) send an $\textsc{epoch-completed}$ message for $e^*$ (line~\ref{line:broadcast_epoch_over}), (4) collect $2f+1$ $\textsc{epoch-completed}$ messages for $e^*$ (line~\ref{line:receive_epoch_over}), and, finally, (5) enter $e^* + 1$ (lines~\ref{line:update_epoch_1},~\ref{line:sync_timer_measure},~\ref{line:sync_timer_expires} and~\ref{line:start_view_2}), resulting in a contradiction.
Note that, if $e^* = 1$, no \textsc{enter-epoch} message is sent: all correct processes enter $e^* = 1$ once they start executing \rare (line~\ref{line:start_view_1}).
% Therefore, there is no ``greatest'' epoch. 
% The lock step also proves that there are no ``gaps'' in epochs, i.e., any epoch $e'$ such that $1 \leq e' \leq e^*$ is entered by a correct process.
% xat a time $t_{e'} \leq t_{e^*}$.
% Thus, every epoch $e \geq 1$ is eventually entered by a correct process.
% We refer to the first time a correct process enters an epoch $e$ as $t_e$.

\smallskip
We now define two epochs: $e_{\mathit{max}}$ and $e_{\mathit{final}} = e_{\mathit{max}} + 1$.
These two epochs are the main protagonists in the proof of correctness and complexity of \rare.

\smallskip
\noindent \textbf{Definition of $\boldsymbol{e_{\mathit{max}}}$:}
\emph{Epoch $e_{\mathit{max}}$ is the greatest epoch entered by a correct process before $\mathit{GST}$; if no such epoch exists, $e_{\mathit{max}} = 0$.\footnote{Epoch $0$ is considered as a special epoch. Note that $0 \notin \mathsf{Epoch}$, where $\mathsf{Epoch}$ denotes the set of epochs (see \Cref{subsection:rare}).}}

\smallskip
\noindent \textbf{Definition of $\boldsymbol{e_{\mathit{final}}}$:} \emph{Epoch $e_{\mathit{final}}$ is the smallest epoch first entered by a correct process at or after $\mathit{GST}$. Note that $\mathit{GST} \leq t_{e_{\mathit{final}}}$. Moreover, $e_{\mathit{final}} = e_{\mathit{max}} + 1$ (by Result 1).}

\smallskip
\noindent \textbf{Result 3:} \emph{For any epoch $e \geq e_{\mathit{final}}$, no correct process broadcasts an \textsc{epoch-completed} message for $e$ (line~\ref{line:broadcast_epoch_over}) before time $t_e + \mathit{epoch\_duration}$, where $\mathit{epoch\_duration} = (f + 1) \cdot \mathit{view\_duration}$.}
\smallskip
\\ This statement is a direct consequence of the fact that, after $\mathit{GST}$, it takes exactly $\mathit{epoch\_duration}$ time for a process to go through $f+1$ views of an epoch; local clocks do not drift after $\mathit{GST}$.
Specifically, the earliest a correct process can broadcast an \textsc{epoch-completed} message for $e$ (line~\ref{line:broadcast_epoch_over}) is at time $t_e + \mathit{epoch\_duration}$, where $t_e$ denotes the first time a correct process enters epoch $e$.
% receive either (1) an $\textsc{enter-epoch}$ message for an epoch greater than $e_{\mathit{final}}$, or (2) $2f+1$ $\textsc{epoch-completed}$ messages for an epoch $\geq e_{\mathit{final}}$ is after time $t_{e_{\mathit{final}}} + \mathit{epoch\_duration}$.
% Hence, no correct process enters an epoch greater than $e_{\mathit{final}}$ by time $t_{e_{\mathit{final}}} + \mathit{epoch\_duration}$.
% $t_{e + 1} > t_e + \mathit{epoch\_duration}$.
% For any epoch $e: t_e \geq \mathit{GST}$, we have that $t_{e+1} > t_e + \mathit{epoch\_duration}$.

\smallskip
\noindent \textbf{Result 4:} \emph{Every correct process enters epoch $e_{\mathit{final}}$ by time $t_{e_{\mathit{final}}} + 2\delta$.} 
\smallskip
\\ Recall that the first correct process enters $e_{\mathit{final}}$ at time $t_{e_{\mathit{final}}}$. 
If $e_{\mathit{final}} = 1$, all correct processes enter $e_{\mathit{final}}$ at $t_{e_{\mathit{final}}}$.
Otherwise, by time $t_{e_{\mathit{final}}} + \delta$, all correct processes will have received an \textsc{enter-epoch} message for $e_{\mathit{final}}$ and started the $\mathit{dissemination\_timer}_i$ with $epoch_i = e_{\mathit{final}}$ (either lines~\ref{line:update_epoch_1},~\ref{line:sync_timer_measure} or~\ref{line:update_epoch_2},~\ref{line:sync_timer_measure_2}).
By results 1 and 3, no correct process sends an \textsc{epoch-completed} message for an epoch $\geq e_{\mathit{final}}$ (line~\ref{line:broadcast_epoch_over}) before time $t_{e_{\mathit{final}}} + \mathit{epoch\_duration}$, which implies that the $\mathit{dissemination\_timer}$ will not be cancelled.
Hence, the $\mathit{dissemination\_timer}$ will expire by time $t_{e_{\mathit{final}}} + 2\delta$, causing all correct processes to enter $e_{\mathit{final}}$ by time $t_{e_{\mathit{final}}} + 2\delta$.
% For an epoch $e: t_e \geq \mathit{GST}$, all correct processes will enter $e$ in the time period $[t_e, t_e + 2\delta]$, i.e., within a maximum delay of $2\delta$ of each other. 

\smallskip
\noindent \textbf{Result 5:} \emph{In every view of $e_{\mathit{final}}$, processes overlap for (at least) $\Delta$ time. In other words, there exists a synchronization time $t_s \leq t_{e_{\mathit{final}}} + \mathit{epoch\_duration} - \Delta$.}
\smallskip
\\ By Result 3, no future epoch can be entered before time $t_{e_{\mathit{final}}} + \mathit{epoch\_duration}$.
% Considering the minimum duration of an epoch $e: t_e \geq \mathit{GST}$, no future epoch can be entered by time $t_e + \mathit{epoch\_duration}$. 
This is precisely enough time for the first correct process (the one to enter $e_{\mathit{final}}$ at $t_{e_{\mathit{final}}}$) to go through all $f+1$ views of $e_{\mathit{final}}$, spending $\mathit{view\_duration}$ time in each view.
Since clocks do not drift after $\mathit{GST}$ and processes spend the same amount of time in each view, the maximum delay of $2\delta$ between processes (Result 4) applies to every view in $e_{\mathit{final}}$.
Thus, all correct processes overlap with each other for (at least) $\mathit{view\_duration} - 2\delta = \Delta$ time in every view of $e_{\mathit{final}}$.
As the $\mathsf{leader}(\cdot)$ function is round-robin, at least one of the $f+1$ views must have a correct leader.
Therefore, synchronization must happen within epoch $e_{\mathit{final}}$, i.e., there is a synchronization time $t_s$ such that $t_{e_{\mathit{final}}} + \Delta \leq t_s + \Delta \leq t_{e_{\mathit{final}}} + \mathit{epoch\_duration}$.

% \smallskip
% \noindent \textbf{The greatest epoch before $\boldsymbol{\mathit{GST}}$.}  
% We define $e_{\mathit{max}} \geq 0$ as the greatest epoch entered by a correct process before $\mathit{GST}$, i.e., at a time $t_{e_{\mathit{max}}} < \mathit{GST}$ (if $\mathit{GST} = 0$, we define $e_{\mathit{max}} = 0$).

% \smallskip
% \noindent \textbf{The first new epoch after $\boldsymbol{\mathit{GST}}$.} We define $e_{\mathit{final}} \geq 1$ as the smallest epoch first entered by a correct process at or after $\mathit{GST}$, i.e., at a time $t_{e_{\mathit{final}}} \geq \mathit{GST}$.
% Note that $e_{\mathit{final}} = e_{\mathit{max}} + 1$.

\smallskip
\noindent \textbf{Result 6:} $t_{e_\mathit{final}} \leq \mathit{GST} + \mathit{epoch\_duration} + 4\delta$\emph{.}
\smallskip
\\ If $e_{\mathit{final}} = 1$, all correct processes started executing \rare at time $\mathit{GST}$.
Hence, $t_{e_{\mathit{final}}} = \mathit{GST}$.
Therefore, the result trivially holds in this case.

Let $e_{\mathit{final}} > 1$; recall that $e_{\mathit{final}} = e_{\mathit{max}} + 1$.
(1) By time $\mathit{GST} + \delta$, every correct process receives an \textsc{enter-epoch} message for $e_{\mathit{max}}$ (line~\ref{line:receive_epoch_over_complete}) as the first correct process to enter $e_{\mathit{max}}$ has broadcast this message before $\mathit{GST}$ (line~\ref{line:broadcast_epoch_over_complete}).
Hence, (2) by time $\mathit{GST} + 2\delta$, every correct process enters $e_{\mathit{max}}$.\footnote{If $e_{\mathit{max}} = 1$, every correct process enters $e_{\mathit{max}}$ by time $\mathit{GST}$.}
Then, (3) every correct process broadcasts an \textsc{epoch-completed} message for $e_{\mathit{max}}$ at time $\mathit{GST} + \mathit{epoch\_duration} + 2\delta$ (line~\ref{line:broadcast_epoch_over}), at latest.
(4) By time $\mathit{GST} + \mathit{epoch\_duration} + 3\delta$, every correct process receives $2f + 1$ \textsc{epoch-completed} messages for $e_{\mathit{max}}$ (line~\ref{line:receive_epoch_over}), and triggers the $\mathsf{measure}(\delta)$ method of $\mathit{dissemination\_timer}$ (line~\ref{line:sync_timer_measure}).
Therefore, (5) by time $\mathit{GST} + \mathit{epoch\_duration} + 4\delta$, every correct process enters $e_{\mathit{max}} + 1 = e_{\mathit{final}}$.
\Cref{fig:raresync_proof} depicts this scenario.

Note that for the previous sequence of events \emph{not} to unfold would imply an even lower bound on $t_{e_{\mathit{final}}}$: a correct process would have to receive $2f+1$ \textsc{epoch-completed} messages for $e_{\mathit{max}}$ or an \textsc{enter-epoch} message for $e_{\mathit{max}} + 1 = e_{\mathit{final}}$ before step (4) (i.e., before time $\mathit{GST} + \mathit{epoch\_duration} + 3\delta$), thus showing that $t_{e_{\mathit{final}}} < \mathit{GST} + \mathit{epoch\_duration} + 4\delta$.
% Due to the minimum duration of $e$, messages for epochs greater than $e$ could not have been received before $t_e$.


% For any epoch $e: t_e \geq \mathit{GST}$, we have that $t_e - \max(t_{e-1}, \mathit{GST}) \leq \mathit{epoch\_duration} + 4\delta$.
% Let $t_0 = 0$.
% Hence, for $e=1$, the previous statement is true.
% By contradiction, suppose that the previous statement is not true for $e>1: t_e \geq \mathit{GST}$.
% % , suppose by contradiction that this is not the case. 
% First, notice that having $t_{e-1} < \mathit{GST}$ or having $t_{e-1} = \mathit{GST}$ is identical: in the worst-case, a single correct process enters $e-1$ at $t_{e-1}$ and none of the other processes receive the required messages to enter $e-1$ before $\mathit{GST} + \delta$.
% Without loss of generality, we consider $t_{e-1} \geq \mathit{GST}$.
% Combining the previous results, every correct process will have at most (1) entered $e-1$ by time $t_{e-1} + 2\delta$, (2) sent an \textsc{epoch-completed} message for $e-1$ one $\mathit{epoch\_duration}$ later, (3) received $2f+1$ \textsc{epoch-completed} messages for $e-1$ one $\delta$ later and, finally, (4) entered $e$ one $\delta$ later.
% Summing up, all correct processes will enter $e$ by time $t_e \leq t_{e-1} + \mathit{epoch\_duration} + 4\delta$, which contradicts the assumption.
% Note that for the previous sequence of events \emph{not} to unfold would also imply a contradiction: a correct process would have to receive $2f+1$ \textsc{epoch-completed} messages for $e-1$ or an \textsc{enter-epoch} message for $e$ before step (3), which would imply an even lower $t_e$ bound.
% Due to the minimum duration of $e$, messages for epochs greater than $e$ could not have been received before $t_e$.

\iffalse
This has an important corollary: any epoch $e$ first entered at time $t_e \geq \mathit{GST}$, which is when process timers are first guaranteed to be accurate, has a minimum duration of $(f + 1) \cdot view\_duration = epoch\_duration$, i.e., any epoch $e'$ greater than $e$ must be entered a time $t_{e'} \geq t_e + epoch\_duration$. 
Before $t_e + epoch\_duration$, no $\textsc{enter-epoch}$ message for a greater epoch can be sent.
\fi

%\smallskip
%\noindent \textbf{Minimum epoch duration after $\mathit{GST}$}.
\iffalse
\smallskip

We now introduce two important concepts, $e_{\mathit{max}}$ and $e_{\mathit{final}}$.

\smallskip
\noindent \textbf{The greatest epoch before \textit{GST}}. We define $e_{\mathit{max}} \geq 0$ as the greatest epoch entered by a correct process before $\mathit{GST}$, i.e., at a time $t_{e_{\mathit{max}}} < \mathit{GST}$ (if $\mathit{GST} = 0$, we define $e_{\mathit{max}} = 0$).

\iffalse
\smallskip
The first result related to $e_{\mathit{max}}$ says that, for any epoch $e' > e_{\textit{max}} + 1$, $e'$ can neither be entered by a correct process nor can any associated $\textsc{enter-epoch}$ message be sent before time $t_{e'} \geq t_{e_{\textit{max}} + 1} + \textit{epoch\_duration} \geq \mathit{GST} + \textit{epoch\_duration}$. 
Otherwise we would reach a contradiction with the corollary of the lock step since, by definition of $e_{max}$, we would have $t_{e_{\textit{max}} + 1} \geq \mathit{GST}$ and the corollary would apply.
This result ensures that correct processes will not get ``stuck'' receiving $\textsc{enter-epoch}$ messages faster than they can enter epochs, and will eventually enter \emph{some} epoch after $\mathit{GST}$.
\fi

\smallskip
\noindent \textbf{The first new epoch after \textit{GST}}. We define $e_{\mathit{final}} \geq 1$ as the smallest epoch first entered by a correct process at or after $\mathit{GST}$, i.e., at a time $t_{e_{\mathit{final}}} \geq \mathit{GST}$.

%There are a few important results related to $e_{\mathit{max}}$ and $e_{\mathit{final}}$. 

%The second result is that some correct process will enter $e_{max} + 1$ by time $t_{e_{\textit{max}} + 1} \leq \mathit{GST} + \textit{epoch\_duration}$. By 

\smallskip

Notice that, combining the definition of $e_{\mathit{max}}$ (which implies $t_{e_{\mathit{max}}} \geq \mathit{GST}$) and due to the the minimum duration of an epoch after $\mathit{GST}$, we get $e_{\mathit{final}} = e_{\mathit{max}} + 1$.
\fi

\smallskip
\noindent \textbf{Latency:} \emph{Latency complexity of \rare is $O(f)$}. 
\smallskip
\\ By Result 5, $t_s \leq t_{e_{\mathit{final}}} + \mathit{epoch\_duration} - \Delta$.
By Result 6, $t_{e_{\mathit{final}}} \leq \mathit{GST} + \mathit{epoch\_duration} + 4\delta$.
Therefore, $t_s \leq \mathit{GST} + \mathit{epoch\_duration} + 4\delta + \mathit{epoch\_duration} - \Delta = \mathit{GST} + 2\mathit{epoch\_duration} + 4\delta - \Delta$.
Hence, $t_s + \Delta - \mathit{GST} \leq 2\mathit{epoch\_duration} + 4\delta = O(f)$.
% Since synchronization happens at every epoch after $\mathit{GST}$, it also happens at $e_{\mathit{final}}$, with $t_s + \Delta \leq t_{e_{\mathit{final}}} + \mathit{epoch\_duration}$.
% Due to the maximum duration of an epoch after $\mathit{GST}$, we get $t_{e_{\mathit{final}}} - \mathsf{max}(t_{e_{\mathit{max}}}, \mathit{GST}) = t_{e_{\mathit{final}}} - \mathit{GST} \leq \mathit{epoch\_duration} + 4\delta$.
% Combining the two results, we get the maximum latency of \rare: $t_s + \Delta \leq 2\cdot\mathit{epoch\_duration} + 4\delta = O(f)$.

\smallskip
\noindent \textbf{Communication:} \emph{Communication complexity of \rare is $O(n^2)$}. 
\smallskip
\\ Roughly speaking, every correct process will have entered $e_{\mathit{max}}$ (or potentially $e_{\mathit{final}} = e_{\mathit{max}} + 1$) by time $\mathit{GST} + 2\delta$ (as seen in the proof of Result 6).
From then on, it will enter at most one other epoch ($e_{\mathit{final}}$) before synchronizing (which is completed by time $t_s + \Delta$).
As for the time interval $[\mathit{GST}, \mathit{GST}+2\delta)$, due to $\mathit{dissemination\_timer}$'s interval of $\delta$, a correct process can enter (at most) two other epochs during this period.
% , e.g., at $t_1 = \mathit{GST}$ and $t_2 = \mathit{GST} + \delta$, or $t_1 < \mathit{GST}$ and $t_2 \in (\mathit{GST}, \mathit{GST} + 2\delta)$.
Therefore, a correct process can enter (and send messages for) at most $O(1)$ epochs between $\mathit{GST}$ and $t_s + \Delta$.
The individual communication cost of a correct process is bounded by $O(n)$ words per epoch: $O(n)$ \textsc{epoch-completed} messages (each with a single word), and $O(n)$ \textsc{enter-epoch} messages (each with a single word, as a threshold signature counts as a single word).
Thus, the communication complexity of \rare is $O(n^2) = O(1) \cdot O(n) \cdot n$. %\ayaz{minor, can ignore. I think it looks better if we reverse the equation, i.e $O(1) \cdot O(n) \cdot n = O(n^2)$}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.2]{figures/raresync_proof.png}
    \caption{Worst-case latency of \rare: $t_s + \Delta - \mathit{GST} \leq 2\mathit{epoch\_duration} + 4\delta$.}
    \label{fig:raresync_proof}
\end{figure}

\smallskip
The formal proof of the following theorem is delegated to \Cref{section:appendix_rare}.

\begin{theorem}
\rare is a partially synchronous view synchronizer with (1) $O(n^2)$ communication complexity, and (2) $O(f)$ latency complexity.
\end{theorem}

\iffalse
JOVAN
\subsection{Drawbacks of \rare} \label{subsection:drawbacks}

In this subsection, we discuss some drawbacks of \rare.

\smallskip
\noindent \textbf{Adaptiveness.}
The first drawback of \rare is that it is not \emph{adaptive} i.e., its complexity does not depend on the \emph{actual} number $b$, but rather on the upper bound $f$, of Byzantine processes.
% It is valuable to obtain complexity which depends on the \emph{actual} number $b$ of Byzantine processes instead of a bound $f$ on this number $b$. 
% This property called adaptiveness (or early-stopping for the latency) is not ensured by our protocol. 
Let us illustrate why \rare is not latency-adaptive.
Consider a scenario $S$ in which all processes are correct; we separate them into three disjoint groups: (1) group $A$, with $|A| = f$, (2) group $B$, with $|B| = f$, and (3) group $C$, with $|C| = f + 1$.
At $\mathit{GST}$, group $A$ is in the first view of epoch $e_{\mathit{max}}$, group $B$ is in the second view of $e_{\mathit{max}}$, and group $C$ is in the third view of $e_{\mathit{max}}$.\footnote{Recall that $e_{\mathit{max}}$ is the greatest epoch entered by a correct process before $\mathit{GST}$; see \Cref{subsection:rare_proof_sketch}.}
Unfortunately, it is impossible for processes to synchronize in epoch $e_{\mathit{max}}$.
Hence, they will need to wait for the end of epoch $e_{\mathit{max}}$ in order to synchronize in the next epoch: thus, the latency is $O(f)$ (since $e_{\mathit{max}}$ has $f + 1$ views) and the communication is $O(n^2)$ (because of the ``all-to-all'' communication at the end of $e_{\mathit{max}}$).
In contrast, the view synchronizer given in~\cite{Naor2020} achieves $O(b)$ latency and $O(b \cdot n)$ communication in the same scenario $S$.
 
% Indeed, we can imagine a scenario $S$ where at GST, the correct processes are partitioned in 3 groups of $f$ processes that are respectively in view $1$, $2$ and $3$ of the same epoch $e_{max}$. Then they will perform $O(f)$ views of epoch $e_{max}$ before triggering the view synchronization of epoch $e_{max + 1}$ and eventually agree on a common value, leading to a worst-case latency complexity of $O( f)$ (and a worst-case communication complexity of $O(f \cdot n)$) . In the same scenario $S$, a protocol that synchronize at each view, like in \cite{ Naor2020}, will perform $O(b)$ views before agreeing on a common value , leading to a worst-case latency complexity of $O(
% b)$ (and a worst-case communication complexity of $O(b^2 \cdot n)$) .

\smallskip
\noindent \textbf{Expected complexity.}
The second drawback of \rare is that its \emph{expected complexity} is the same as its worst-case complexity.
Namely, the expected complexity considers a weaker adversary which does not have a knowledge of the $\mathsf{leader}()$ function. %$\matsfh{leader}()$ function.
Therefore, this adversary cannot corrupt $f$ processes that are scheduled to be leaders right after $\mathit{GST}$.

As the previously introduced scenario $S$ does not include any Byzantine process, we can analyze it for the expected complexity of \rare.
Therefore, the expected latency complexity of \rare is $O(f)$ and the expected communication complexity of \rare is $O(n^2)$.
On the other hand, the view synchronizer given in~\cite{Naor2020} achieves $O(1)$ expected latency complexity and $O(n)$ expected communication complexity.


% Our protocol is designed to optimize worst-case complexity only, but neglects expected complexity, where the adversary does not choose the Byzantine processes according to the order of leaders. Again, because of scenario $S$, the expected complexity is the same than the worst-case complexity, that is an expected latency complexity of $O(f)$ and an expected communication complexity of $O(f \cdot n)$. In the same scenario, protocol from $\cite{Naor2020}$ synchronize a $O(1)$ expected number of times, with a $O(n)$ expected communication complexity per view synchronization, leading to a $O(1)$ expected latency complexity and a $O(n)$ expected communication complexity. 

\smallskip
\noindent \textbf{Clock drift tolerance.}
The final drawback of \rare is that its latency is susceptible to clock drifts.
Namely, let $\phi > 1$ denote the bound on clock drifts.\footnote{Our system model assumes that $\phi = 1$ after $\mathit{GST}$.}
To accommodate for the clock drifts, the duration of a view increases. 
Namely, the duration of $i$-th view in an epoch becomes $\phi^i \cdot \mathit{view\_duration}$ (instead of only $\mathit{view\_duration}$).
Thus, the latency complexity of \rare becomes $O(f \cdot \phi^f)$.
In practice, $\phi$ is a relatively small parameter.\footnote{For reference, a clock drift value of $200$ parts per million ($\phi = 1.0002$) is already considered high~\cite{Kleppmann2014}. For scale, it would take $f > 50.000$ before $\phi^f \sim f$, at which point $O(f)$ latency is already impractical regardless. With atomic clocks, we can even get $\phi = 10^{-13}$: it would take 32 million years before the clock drifts by a single second. }
In contrast with \rare, the view synchronizer of Naor and Keidar~\cite{Naor2020} achieves $O(f \cdot \phi)$ latency while tolerating clock drifts.
JOVAN
\fi


% the duration of a view must be multiplied by $\phi$, i.e., the new duration of a view becomes $$

% Our system model assumes that there is no clock drift after $\mathit{GST}$.
% % supposes that after GST, there is no clock drift, i.e. the real time is available to correct processes. It is legitimate to ask what happen if this assumption does not hold. 


% Let us investigate a less accomodating model where after GST, there exists a known bound $c > 1$ on clock drift. Without loss of generality, we assume that every correct process measures real time with a clock drift in $[1,c]$. Hence, if a correct process sets its timer to $c \cdot s$ seconds, when its timer expires, $s' \in [s, c \cdot s]$ real time seconds have elapsed.
% The algorithm \ref{algorithm:synchronizer} has to be slightly modified as follows: line \ref{line:view_timer_measure_without_msg_exchange} of algorithm \ref{algorithm:synchronizer}  becomes $view\_timer_i$.measure$(c^{v} \cdot view\_duration$).
% Thus, if we want to tolerate clock drift after GST, synchronizing at each epoch only leads to a worst-case latency complexity of $O(f \cdot c^{f})$, while synchronizing at each view, like in \cite{Naor2020}, leads to a worst-case latency complexity of $O(f \cdot c)$.

%where $k_{v}$ is an accurate coefficient, depending on view $v$ and clock drift bound $c$, to maintain the necessary and sufficient overlap of $\Delta$ time at each view after first epoch synchronization after GST. In our case, setting $\forall v \in [1,f+1], k_{v} = c^{v}$ is necessary and sufficient to maintain the overlap (we fix $k_{0} = 0$). Indeed, for any $v \in [0,f+1]$, after $\tau_{v} = 2\delta + 10 \delta \cdot \sum_{i \in [1,v]} k_{i}$ real time, the slowest process can enter in view $v+1$, while for any $v' \in [0,f]$, after $\tau'_{v'} = 10 \delta \cdot \sum_{i \in [1,v']} \frac{k_{i}}{c}$ real time, the faster correct process can enter in view $v'+1$. To maintain the overlap, we want $\forall v \in [0,f]$, $\tau'_{v+1}- \tau_{v} \geq \Delta$. This lead us to $\forall v \in [0,f]$, $k_{v+1} \geq c +  (c-1) \cdot \sum_{i \in [1,v]} k_i $ and finally $\forall r \in [1,f+1]$, $k_{v} \geq c^{v}$ after an immediate induction. Thus, if we want to tolerate clock drift after GST, synchronizing at each epoch only leads to a worst-case latency complexity of $O(10 \delta \cdot c^{f})$, while synchronizing at each view, like in \cite{Naor2020}, leads to a worst-case latency complexity of $O(10 \delta \cdot c)$.

%%%%remove table
\iffalse
\begin{table}[]
\begin{tabular}{|l|ll|ll|ll|}
\hline
Protocols  & \multicolumn{2}{l|}{Complexity with clock drift}                                                                                                                & \multicolumn{2}{l|}{Adaptative Complexity}                                                         & \multicolumn{2}{l|}{Expected Complexity}                                                           \\ \hline
           & \multicolumn{1}{l|}{Latency}                                                                                   & Communication                                  & \multicolumn{1}{l|}{Latency}                                         & Communication               & \multicolumn{1}{l|}{Latency}                                         & Communication               \\ \hline
This paper & \multicolumn{1}{l|}{$O( f \cdot c^f)$} & $O(f \cdot n)$                    & \multicolumn{1}{l|}{$O(f)$} & $O(f \cdot n)$ & \multicolumn{1}{l|}{$O(f)$} & $O(f \cdot n)$ \\ \hline
\cite{Naor2020}       & \multicolumn{1}{l|}{$O(b \cdot c)$}                    & $O(b^2 \cdot n)$ & \multicolumn{1}{l|}{$O(b)$} & $O(b^2 \cdot n)$ & \multicolumn{1}{l|}{$O(1)$}                        & $O(n)$                        \\ \hline
\end{tabular}
\caption{Comparison between our solution and state-of-art solution \cite{Naor2020}. The only improvement is for worst-case communication complexity where we reach the Dolev-Reischuk bound}. We also meet the optimal worst-case latency complexity when there is no clock drift after GST.
\end{table}
\fi
%%%end remove table

\iffalse
Notice that, assuming $e_{\mathit{final}}$ exists, $e_{\mathit{final}} = e_{\mathit{max}} + 1$.
Indeed, if $\mathit{GST} = 0$, this is trivially verified: $e_{\mathit{max}} = 0$ (by definition) and processes immediately enter epoch 1 (line~\ref{line:start_view_1}), hence $e_{\mathit{final}} = 1 = e_{\mathit{max}} + 1$.
Otherwise we have that $\mathit{GST} > 0$ and $e_{\mathit{max}} \geq 1$ (line~\ref{line:start_view_1}).
As a result of the lock step, processes starting at epoch 1 (line~\ref{line:start_view_1}), and by definition of $e_{\mathit{max}}$, any epoch $e'$ such that $1 \leq e' \leq e_{\mathit{max}}$ has been entered by some correct process at time $t' \leq t_{e_{\mathit{max}}} < \mathit{GST} \leq t_{e_{\mathit{final}}}$. 
Therefore, $e_{\mathit{final}} > e_{\mathit{max}}$. Now suppose by contradiction that $e_{\mathit{final}} > e_{\mathit{max}} + 1$. 
By the lock step, $e_{\mathit{max}} + 1 < e_{\mathit{final}}$ must have been entered before and, by definition of $e_{\mathit{max}}$, it was entered at time $t_{e_{\mathit{max}} + 1} \geq \mathit{GST}$.
This implies that $e_{\mathit{final}} = e_{\mathit{max}} + 1$.
\fi

\iffalse

\noindent \textbf{Latency of \rare}.  We show that $e_{final}$ exists and $t_{e_{\textit{final}}} \leq \mathit{GST} + \textit{epoch\_duration} + 4\delta$.

\smallskip

We proceed by contradiction. Suppose that by time $t^* > \mathit{GST} + \textit{epoch\_duration} + 4\delta$ no correct process has entered $e_{\mathit{final}}$.
Notice that receiving an $\textsc{enter-epoch}$ message for $e \geq e_{\mathit{final}}$ by time $t^* - \delta$ results in a contradiction.
By the lock step corollary, no correct process will enter or receive an $\textsc{enter-epoch}$ message for $e > e_{\mathit{final}}$ before $t^* + \textit{epoch\_duration}$.
Furthermore, if a correct process receives an $\textsc{enter-epoch}$ message for $e = e_{\mathit{final}}$ by $t^* - \delta$, its dissemination timer will expire after $\delta$ time and the process will enter $e_{\mathit{final}}$ by $t^*$, which contradicts the assumption. Keeping these two facts in mind, we have that:
\begin{compactitem}
    \item Every correct process enters $e_{\mathit{max}}$ by $\mathit{GST} + 2\delta$.
    If $e_{\mathit{max}} = 1$, this is trivially true. 
    Otherwise, $e_{\mathit{max}} > 1$ and every correct process receives an $\textsc{enter-epoch}$ message for $e_{\mathit{max}}$ by $\mathit{GST} + \delta$.
    All correct processes enter $e_{\mathit{max}}$ by $\mathit{GST} + 2\delta$ after their dissemination timer expires (line~\ref{line:sync_timer_expires}).
    \item Every correct process sends an $\textsc{epoch-completed}$ message by $\mathit{GST} + \textit{epoch\_duration} + 2\delta$.
    After entering $e_{\mathit{max}}$, each correct process goes through every view in $e_{\mathit{max}}$ and then sends an $\textsc{epoch-completed}$ for $e$.
    Since clocks do not drift after $\mathit{GST}$, this takes at most $\mathit{epoch\_duration}$ time.
    \item \textit{Every correct process receives $2f+1$ $\textsc{epoch-completed}$ messages by $\mathit{GST} + \textit{epoch\_duration} + 3\delta$}, setting its $epoch_i$ variable to $e_{\textit{max}} + 1 = e_{\mathit{final}}$.
    From then on, it ignores any $\textsc{enter-epoch}$ message for $e_{\mathit{final}}$ (line~\ref{line:receive_epoch_over_complete}).
    \item Finally, each correct process enters $e_{final}$ by time $t^* = \mathit{GST} + \textit{epoch\_duration} + 4\delta$ after its dissemination timer expires.
    This contradicts the assumption.
\end{compactitem}

\smallskip

\noindent \textbf{Maximum delay between processes in $\mathbf{e_{\textit{final}}}$}. Every correct process enters $e_{\mathit{final}}$ within $[t_{e_{\textit{final}}}, t_{e_{\textit{final}}} + 2\delta]$, i.e., with a maximum delay of $2\delta$. The first time a correct process enters $e_{\mathit{final}}$ is at time $[t_{e_{\textit{final}}}$, by definition. 

\smallskip

\noindent \textbf{Synchronization is reached in $\mathbf{e_{\textit{final}}}$}.

\smallskip

\noindent \textbf{Latency and Communication complexities of \rare}.

The protocol increments a counter variable $global\_view$ and repeatedly triggers $\texttt{advance}(global\_view)$ (line~\ref{line:start_view_1}, \ref{line:start_view_without_msg_exchange}, \ref{line:start_view_2}) to enforce the core protocol to advance in the view $global\_view$.
The views are partitioned into epochs, that are set of $f+1$ consecutive views. Epoch 1 is the set of views $1, 2, ..., f+1$, epoch 2 is the set of views $f+2, f+3, ..., f+2$, etc. We say that process $P_i$ enters in view $v$ of epoch $e$ at time $t$ if it triggers $\texttt{advance}(global\_view)$ at time $t$ for variables $global\_view = (e-1) \cdot (f+1) + v$. If $v=1$, we say that $P_i$ enters in epoch $e$ (line~\ref{line:start_view_1}, \ref{line:start_view_2}). 
Every time a correct process enters in a view $v$, it sets its timer $view\_timer$ to $view\_duration$ (line~\ref{line:view_timer_measure_first_view}, \ref{line:view_timer_measure_without_msg_exchange}, \ref{line:view_timer_measure}). Then, by default (if it does not receive special messages), it waits for  $view\_timer$ expiration (line~\ref{line:rule_view_expired}), enter in next view (line \ref{line:start_view_without_msg_exchange}) and repeat that procedure again until it reach a new epoch. 
When the timer of correct process $P_i$ expires for last view of epoch $e$, $P_i$ informs the other processes that it terminated the epoch $e$ by broadcasting an $\textsc{epoch-over}$ message  for epoch $e$ with its share-signature (line~\ref{line:broadcast_epoch_over}). At this moment, process $P_i$ does not want to make progress alone. This is why, before starting next epoch, he waits for some special messages (line~\ref{line:receive_epoch_over}, \ref{line:receive_epoch_over_complete}) that cannot be computed if less than $f+1$  correct processes did not visit the epoch $e$. In fact, the reception of these special messages is a necessary and sufficient condition to start a new epoch $e'>e$, even if the current epoch $e$ is not over for $P_i$ but over for $2f+1$ processes, and so at least for $f+1$ correct processes.

Upon the reception of $2f+1$ share-signed $\textsc{epoch-over}$ messages for epoch $e$ with valid share-signatures (line~\ref{line:receive_epoch_over}), correct process $P_i$ combines the share-signatures to obtain a threshold signature (line \ref{line:combine-signatures}), wait $\delta$ time (line~\ref{line:sync_timer_measure} and \ref{line:sync_timer_expires}) to check if it does not receive some special messages for an higher epoch,  broadcasts an $\textsc{epoch-over-complete}$ message for epoch $e$ with the attached threshold signature (line~\ref{line:broadcast_epoch_over_complete}) and then advances to the epoch $e+1$ (line~\ref{line:start_view_2}). 
In the same way, upon the reception of a  $\textsc{epoch-over-message}$ message for epoch $e$ with valid threshold-signature (line~\ref{line:receive_epoch_over_complete}), correct process $P_i$ wait $\delta$ time (line~\ref{line:sync_timer_measure_2} and \ref{line:sync_timer_expires}) to check if it does not receive some special messages for an higher epoch, re-broadcast the same $\textsc{epoch-over-complete}$ message for epoch $e$ with the same attached threshold signature  (line~\ref{line:broadcast_epoch_over_complete}) and then advances to the epoch $e+1$ (line~\ref{line:start_view_2}). 
Waiting $\delta$ time (line~\ref{line:sync_timer_measure} or \ref{line:sync_timer_measure_2} and \ref{line:sync_timer_expires}) allows to bound the communication-complexity after GST, to not send an unbounded number of $\textsc{epoch-over}$ and $\textsc{epoch-over-complete}$ messages.
\fi





\iffalse
As a corollary, we directly obtain the communication complexity of \name.

\begin{theorem} [Communication complexity]
\name has $O(n^2)$ communication complexity.
\end{theorem}
\begin{proof}
%By time $\mathit{GST} + \delta$, each process receives an \textsc{epoch-over-complete} message for epoch $e_{\mathit{max}} - 1$ . Hence, before time $\mathit{GST} + 3\delta$ each correct process starts either epoch $e_{\mathit{max}}$ or $e_{\mathit{max}} + 1$. Let us explain: a correct process $P_i$ receives an \textsc{epoch-over-complete} message for $e_{\mathit{max}} - 1$ at time $\mathit{GST} + \delta$, sets its $\mathit{sync\_epoch}$ variable to $e_{\mathit{max}}$ and sets $\mathit{sync\_timer}$ to measure $\delta$ time; just before time $\mathit{GST} + 2\delta$, $P_i$ receives an \textsc{epoch-over-complete} message for $e_{\mathit{max}}$, sets its $\mathit{sync\_epoch}$ variable to $e_{\mathit{max}} + 1$ and sets $\mathit{sync\_timer}$ to measure $\delta$ time; therefore, before time $\mathit{GST} + 3\delta$, $P_i$ starts $e_{\mathit{max}} + 1$. Let us fix a correct process $P_i$. By time $\mathit{GST} + 3\delta$, $P_i$ starts either epoch $e_{\mathit{max}}$ or epoch $e_{\mathit{max}} + 1$ (because of the argument given above). By \Cref{lemma:no_process_starts_emax_1}, $P_i$ never starts an epoch greater than $e_{\mathit{max}} + 1$ before synchronization time. During $3\delta$ time period, $P_i$ can be in (at most) $6$ epochs (by \Cref{lemma:within_delta}); afterwards, $P_i$ can be in two epochs ($e_{\mathit{max}}$ and $e_{\mathit{max}} + 1$).
Since it sends at most $O(n)$ words within every epoch (by \Cref{lemma:linear_in_an_epoch}), and that $P_i$ visit at most $O(1)$ epochs between $\mathit{GST}$ and synchronization time (by \Cref{lemma:constant-number-of-epochs-after-GST}), $P_i$ sends at most $O(n)$ words between $\mathit{GST}$ and synchronization time.
Therefore, the communication complexity of \name is indeed $O(n^2)$.
\end{proof}
\fi

\iffalse
*************************************
\subsection{\name}

\smallskip
\noindent \textbf{Composition.}
Finally, \Cref{algorithm:composition} shows how the view core and the view synchronizer components collaborate in order to solve Byzantine consensus.

\begin{algorithm}
\caption{Core + Synchronizer = Byzantine Consensus}
\label{algorithm:composition}
\begin{multicols}{2}
\begin{algorithmic} [1]
\State \textbf{upon} $\mathsf{init}$:
\State \hskip2em $\texttt{Core.}\mathsf{init(}\mathit{proposal}\mathsf{)}$

\smallskip
\State \textbf{upon} $\texttt{Synchronizer.}\mathsf{advance(}v\mathsf{)}$:
\State \hskip2em $\texttt{Core.}\mathsf{start(}v\mathsf{)}$

\columnbreak
\smallskip
\State \textbf{upon} $\texttt{Core.}\mathsf{decide(}v\mathsf{)}$:
\State \hskip2em \textbf{trigger} $\mathsf{decide(}v\mathsf{)}$
\end{algorithmic}
\end{multicols}
\end{algorithm} 

We prove the correctness and the complexity of \Cref{algorithm:composition}.

\begin{theorem} \label{theorem:quad-solves-consensus} \name
(\Cref{algorithm:composition}) solves the Byzantine consensus problem with $O(n^2)$ worst-case communication complexity and $O(f\cdot \delta)$ worst-case latency complexity.
\end{theorem}
\begin{proof}
The safety properties of Byzantine consensus follows directly from the safety properties of the core module. The termination comes from the eventual view synchronization property of the view synchronizer component.
By lemma \ref{lemma:constant-number-of-epochs-after-GST}, no correct process visit more than $O(1)$ epochs.

Since a correct process sends at most $O(n)$ words within every epoch (by \Cref{lemma:linear_in_an_epoch}) of the synchronizer module, and at most $O(n)$ words within every epoch of the core module, by using Hotstuff core protocol, the worst-case communication complexity of \name is $O(n^2)$.

Moreover, the duration of an epoch is $(f+1)\cdot (c_s+2) \cdot \delta$, which means the worst-case latency complexity is $O(f \cdot \delta)$. 
The theorem holds.

For sake of completeness, the pseudo-code of HotStuff can be found in the appendix.

\end{proof}

%% merged into one unique theorem
\iffalse
Finally, we prove the complexity of \Cref{algorithm:composition}.

\begin{theorem}
The communication complexity of \Cref{algorithm:composition} is $\mathit{num\_views} \cdot \mathit{com\_per\_view} + \mathit{sync\_com}$.The latency complexity of \Cref{algorithm:composition} is $\mathit{num\_views} \cdot \mathit{latency\_per\_view} + \mathit{sync\_latency}$.
\end{theorem}

\fi
%merge into one unique theorem

\subsection{Adding strong validity to \name}

The actual \name protocol only ensures weak validity (if all processes are correct and a process decides value $w$, then value $w$ is proposed by a correct process) but does not ensure \emph{strong validity}: If all correct processes propose the same value $w$, then $w$ is decided. In this subsection, we add a groundwork step before \name to obtain \namebis that solves consensus with strong validity, quadratic worst-case communication complexity and linear worst-case latency complexity.

\subsubsection{Implementation of \namebis}

We assume another $(k', n)$-threshold signature scheme~\cite{Libert2016}, where $k' = f + 1$ (and not $2f+1$). In the remaining, \name is used in a black-box fashion, so we use the same names $ShareSign$, $ShareVerify$, $Combine$, $Verify$ for the $(k', n)$-threshold signature without fearing any ambiguity with the $(2f+1, n)$-threshold signature used in \name.

 The basic idea is to propose and accept only values that are \emph{legitimate}, in the sense that deciding one of them cannot violate strong validity. Hence a groundwork is added to know what are the legitimate values. At first view of the groundwork, every correct process send its (signed) proposal. If a process $p$ does not receive $f+1$ times the same proposal, it knows that any value $w$ could be decided safely. A naive solution could consist in broadcasting $2f+1$ signed proposals, s. t. eventually, every correct process knows that any value $w$ could be decided safely. But it would induce a $O(n^3)$ communication complexity. We adapt this idea with some optimization to reach a $O(n^2)$ communication complexity. The groundwork pseudo-code is presented in \ref{algorithm:groundwork} and counts 3 rounds that are presented here.
 \begin{enumerate}
     \item PROPOSAL: every process $i$ send its partially-signed proposal $[PROPOSAL, proposal_i]_{\sigma_i}$ (line \ref{line-gw:bcast-proposal}).
     
     \item ECHO: Upon the reception of $2f+1$ proposals (line \ref{line-gw:proposal-reception}), a process deals with two possible situations:
     \begin{enumerate}
         \item It did not receive more than $f$ times the same proposal (line \ref{line-gw:not-same-proposals}). It knows that any value can be safely decided. To inform other processes, it broadcasts a message $[ECHO, \bot]_{\sigma_i}$ (line \ref{line-gw:claim-not-same-proposals} and \ref{line-gw:bcast-echo}).
         
         \item It received $f+1$ times the same proposal $w$ (line \ref{line-gw:same-proposals}). Potentially, it could be the only legitimate  value to decide. To inform the other processes, it broadcast a message $[ECHO, \sigma]$ where $\sigma$ is the $(f+1)$-threshold signature of message $[PROPOSAL, w]$ (line \ref{line-gw:certify-same-proposals} and \ref{line-gw:bcast-echo}). 
          \end{enumerate}
     
     \item JUSTIFICATION: Upon the reception of $2f+1$ echo messages, a process deals with two possible situations:
     \begin{enumerate}
     \item It receives $f+1$ messages of the form $[ECHO, \bot]_{\sigma_j}$ (line \ref{line-gw:uniform-claim-not-same-proposals}).
     The process knows
     that any value can be safely decided, but now, it can prove it with a reasonable cost. To inform other processes, it broadcasts a message $[JUSTIFICATION, \sigma]$ where $\sigma$
 is the $(f+1)$-threshold signature of message $[ECHO, \bot]$ (line \ref{line-gw:certify-uniform-claim-not-same-proposals} and \ref{line-gw:bcast-justification}). 
 
 \item It does not receive $f+1$ messages of the form $[ECHO, \bot]_{\sigma_j}$. Here again, two possibilities: 
 \begin{enumerate}
     \item it receives $m_x = [ECHO, \sigma_x]$ and $m_y = [ECHO, \sigma_y]$ that justifies two different values $x$ and $y$ (line \ref{line-gw:at-least-two-different proposals}). Since at least two different correct processes proposed two different values, the process knows
     that any value can be safely decided, but now, it can prove it with a reasonable cost. To inform other processes, it broadcasts $[JUSTIFICATION, (m_x, m_y)]$ (line \ref{line-gw:certify-at-least-two-different-proposals} and \ref{line-gw:bcast-justification-2}).
     \item it receives only message of the form $m_w = [ECHO, \sigma_w]$ that justifies $w$ (line \ref{line-gw:all-processes-consider-value-legitimate}) (with $Verify([PROPOSAL,w], \sigma_w)==true$) . In that case, all the correct processes also receive $[ECHO, \sigma_w]$ and thus knows that $w$ can be decided safely. Moreover, it updates its proposal to $w$ before starting \name (line \ref{line-gw:update-proposal-upon-same-proposals}). 
 \end{enumerate}
     \end{enumerate}
     
     \item Later, a message $m$ legitimates a value $w$ iff it is a well-formed JUSTIFICATION message or if $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$. %either (1)  $m = (JUSTIFICATION, \sigma)$ with $Verify([ECHO, \bot], \sigma)$ or 
 %(2)  $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$ or
 %(3) $m = ( JUSTIFICATION, \{m_x, m_y\} )$ with $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ and $x \neq y$. 
 Upon the reception of the first JUSTIFICATION message, it is broadcast in order to ensure uniformity, i. e. if a value is considered legitimate by a correct process, it is considered legitimate by all correct processes by time $GST + \delta$.
     It is worthy to note that if no justification message is sent by a correct process, it means it is in case 3) b) ii) which means that every correct process receives a message $[ECHO, \sigma_w]$  s.t. $Verify([PROPOSAL, w], \sigma_w)$.
 \end{enumerate}
 
 The pseudo-code of \namebis is presented in algorithms \ref{algorithm:groundwork} and \ref{algorithm:wrapper-for-strong-validity}.

\begin{algorithm} 
\caption{GroundWork: Pseudocode for process $P_i$}
\label{algorithm:groundwork}
\begin{algorithmic} [1]

%Sending Phase proposal
\State \textbf{upon} \texttt{start}: \BlueComment{start of the algorithm}

\State \hskip2em $certified \gets \emptyset$

\smallskip

\State \hskip2em $m^p.\mathit{type} \gets PROPOSAL$
\State \hskip2em $m^p.\mathit{proposal} \gets proposal_i$
\State \hskip2em $m^p.\mathit{partial\_sig} \gets \mathit{ShareSign}_i([m^p.\mathit{type}, m^p.\mathit{proposal}])$
\State \hskip2em \texttt{broadcast} $m^p$ \label{line-gw:bcast-proposal}

\smallskip

%%%Rcving Phase proposal
\State \hskip2em \textbf{wait for } $2f + 1$ proposals: $M \gets \{m'|m'.type = PROPOSAL\}$.  \label{line-gw:proposal-reception}
\State \hskip2em \textbf{if } $\exists M' \subset M$, s. t. $\forall m', m'' \in M', m'.\mathit{proposal} = m''.proposal$: \label{line-gw:same-proposals}

\State \hskip4em $m^e.\mathit{cert} \gets Combine(\{m'.\mathit{partial\_sig}| m' \in M'\})$ \label{line-gw:certify-same-proposals}
%\State \hskip4em $proposal_i \gets w$ where $Verify([Proposal, w], m^e.\mathit{cert})$ \label{line-gw:update-proposal-upon-same-proposals}
\State \hskip2em \textbf{else } \label{line-gw:not-same-proposals} 
\State \hskip4em $m^e.\mathit{cert} \gets \bot$ \label{line-gw:claim-not-same-proposals}

\State \hskip2em $m^e.\mathit{type} \gets ECHO$
\State \hskip2em $m^e.\mathit{partial\_sig} \gets ShareSign_i([m^e.\mathit{type}, m^e.\mathit{cert}])$

\State \hskip2em \texttt{broadcast} $m^e$ \label{line-gw:bcast-echo}

\smallskip
%%%
\State \hskip2em \textbf{wait for } $2f + 1$ echo messages: $M \gets \{m'|m'.type = ECHO\}$.
\State \hskip2em \textbf{if } $\exists M' \subset M$, s. t. $\forall m' \in M', m'.\mathit{cert} = \bot$: \label{line-gw:uniform-claim-not-same-proposals}

\State \hskip4em $m^j.\mathit{type} \gets$ $JUSTIFICATION$

\State \hskip4em $m^j.\mathit{justification} \gets$ $Combine(\{m'.\mathit{partial\_sig}| m' \in M'\})$ \label{line-gw:certify-uniform-claim-not-same-proposals}

\State \hskip4em \texttt{broadcast} $m^j$ \label{line-gw:bcast-justification}

\State \hskip2em \textbf{else if}: $\exists m_x, m_y \in M$ s. t. $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ with $x \neq y$ \label{line-gw:at-least-two-different proposals}

\State \hskip4em $m^j.\mathit{type} \gets$ $JUSTIFICATION$

\State \hskip4em $m^j.\mathit{justification} \gets$ $\{m_x, m_y\}$ \label{line-gw:certify-at-least-two-different-proposals}

\State \hskip4em \texttt{broadcast} $m^j$ \label{line-gw:bcast-justification-2}


\State \hskip2em \textbf{else}: \label{line-gw:all-processes-consider-value-legitimate}

\State \hskip4em $proposal_i \gets w$ where  $Verify([PROPOSAL, w], m'.cert)$ for some $m' \in M$ \label{line-gw:update-proposal-upon-same-proposals}

\State \hskip2em \textbf{trigger} \texttt{terminate\_GroundWork}

\smallskip

%%%Uniformity Phase
\State \textbf{upon} first reception of a message $m$ with $m.type = JUSTIFICATION$
\State \hskip2em \texttt{broadcast} $m$ if it is not already done \label{line-gw:forward-justification}

%\smallskip

%\State \textbf{upon} reception of a message $m$ with $m.type = ECHO$ and $Verify([ECHO, x], m.cert)$
%\State \hskip2em $certified \gets certified \cup \{x\}$
%\State \hskip2em \textbf{if} $|certified| \leq 2$:
%\State \hskip4em \texttt{broadcast} $m$

\smallskip
%Utility

\State \textbf{function} \texttt{legitimate}(\texttt{Message} $m$, \texttt{Integer} $w$):
\State \hskip2em \textbf{if} either
\State \hskip4em (1)  $m = (JUSTIFICATION, \sigma)$ with $Verify([ECHO, \bot], \sigma)$ or 
\State \hskip4em (2)  $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$ or
\State \hskip4em (3) $m = ( JUSTIFICATION, \{m_x, m_y\} )$ with $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ and $x \neq y$:
\State \hskip6em \textbf{return} true

\State \hskip2em \textbf{else}
\State \hskip4em \textbf{return} false



\end{algorithmic}
\end{algorithm}

\begin{algorithm} 
\caption{\namebis: Pseudocode for process $P_i$}
\label{algorithm:wrapper-for-strong-validity}
\begin{algorithmic} [1]
\State \texttt{start} GroundWork
\State \textbf{upon} \texttt{terminate\_GroundWork}: \State \hskip2em \texttt{start} \name where a proposal $w$ is ignored in the PREPARE phase of any view iff no message $m$ s. t. $\texttt{legitimate}(m, w)$ has been delivered 
\end{algorithmic}
\end{algorithm}

\subsubsection{Proof of correctness of \namebis}

Here we prove the correctness of the algorithm \namebis.

\begin{lemma}[Validity]\label{lemma:sv-validity}
If all correct processes proposes the same value $w$, then
\begin{enumerate}
    \item every correct process receives (immediately from itself) a message $m = [ECHO, \sigma]$ with $Verify([PROPOSAL, w], \sigma)$
    \item No correct process delivers $M$ s. t. $\texttt{legitimate}(M, x)$ with $x \neq w$
\end{enumerate}
 
\end{lemma}

\begin{proof}
They are at least $2f+1$ broadcast of  messages of the form $[PROPOSAL, w]_{\sigma_j}$ (line \ref{line-gw:bcast-proposal}). Hence, every correct process receives $f+1$ messages of the form $[PROPOSAL, w]_{\sigma_j}$ (line \ref{line-gw:same-proposals}) and hence sends  $ [ECHO, \sigma]$ with $Verify([PROPOSAL, w], \sigma)$ (line \ref{line-gw:certify-same-proposals} and \ref{line-gw:bcast-echo}). This implies the item (1) of the lemma.
Moreover, the $f$ remaining processes cannot neither compute $ [ECHO, \sigma']$ with $Verify([PROPOSAL, x], \sigma')$ with $x \neq w$ nor compute $[JUSTIFICATION, \sigma_{\bot}]$ with $Verify([ECHO, \bot], \sigma_{\bot})$, since the threshold-scheme requires at least $f+1$ different share-signatures. 



\end{proof}

\begin{lemma}[Uniformity]\label{lemma:sv-uniformity}
If a correct process delivers $m$ by time $t$ s. t. $\texttt{legitimate}(m, w)$, then every correct process eventually receives $m'$ s. t. $\texttt{legitimate}(m', w)$ by time $max(GST, t) + \delta$.
\end{lemma}

\begin{proof}
Let $p$ be a correct process that terminates the GroundWork.
Necessarily, $p$ enter either in line \ref{line-gw:uniform-claim-not-same-proposals} or \ref{line-gw:at-least-two-different proposals} or in line \ref{line-gw:all-processes-consider-value-legitimate}. In first case, $p$ broadcast a JUSTIFICATION message (lines \ref{line-gw:certify-uniform-claim-not-same-proposals}and  \ref{line-gw:bcast-justification} or lines \ref{line-gw:certify-at-least-two-different-proposals} and  \ref{line-gw:bcast-justification-2} ) that legitimates all possible values. 
By justification's forwarding  (line \ref{line-gw:forward-justification}), if a justification message is received by a correct process by time $t$, then a justification message is received by each correct process by time $max(GST, t) + \delta$.
The only way to avoid that every correct process obtain a justification message before $GST + \delta$ is if all correct processes enter in line \ref{line-gw:all-processes-consider-value-legitimate}. But it is impossible that two correct processes enter in line \ref{line-gw:all-processes-consider-value-legitimate} for two different values. Hence they enter in line \ref{line-gw:all-processes-consider-value-legitimate} for one unique value $w$, which means they all received a message $m = [ECHO, \sigma_w]$ with $Verify([PROPOSAL, w], \sigma_w)$, which ends the proof.
\end{proof}



\begin{lemma}[Obligation]\label{lemma:sv-obligation}
After GST, for every correct leader $p$, its proposal is not ignored.  
\end{lemma}

\begin{proof}
Case 1: the proposal is its own proposal in \name.

This proposal has been chosen according to received messages in the groundWork algorithm.
$p$ entered either (i) in line \ref{line-gw:uniform-claim-not-same-proposals} or \ref{line-gw:at-least-two-different proposals} or (ii) in line \ref{line-gw:all-processes-consider-value-legitimate}.
In case (i), a JUSTIFICATION message will be received by every correct process by time $GST + \delta$.
In case (ii), the proposal has been updated to the relevant value so that every correct process receives $(ECHO, \sigma_w)$ with $Verify([PROPOSAL, w], \sigma_w)$.

Case 2: its proposal comes from the delivered $2f+1$ VIEW-CHANGE messages.

A VIEW-CHANGE message, encapsulates necessarily a value considered legitimate by at least $f+1$ correct processes by the quorum certificate.  The lemma holds by lemma \ref{lemma:sv-uniformity}.  
\end{proof}

\begin{lemma}[$O(n^2)$ complexity]\label{lemma:sv-complexity}
The communication complexity of the GroundWork algorithm is $O(n^2)$
\end{lemma}

\begin{proof}
Every correct process broadcast only one PROPOSAL message, one ECHO message and at most one JUSTIFICATION message where each message contains no more than ine threshold-signature and no more than share-signature.
\end{proof}

\begin{theorem}[Strong Validity]
 \namebis solves Byzantine consensus with strong validity, $O(n^2)$ communication complexity and $O(f\cdot\delta)$ latency complexity. 
\end{theorem}

\begin{proof}
 The strong validity is ensured by lemma \ref{lemma:sv-validity}. The liveness of the algorithm is preserved by lemma \ref{lemma:sv-obligation}. The quadratic communication complexity is ensured by lemma \ref{lemma:sv-complexity} and theorem \ref{theorem:quad-solves-consensus}.
 The latency complexity is ensured by theorem \ref{theorem:quad-solves-consensus}, since the groundwork only add 3 additional asynchronous rounds.
\end{proof}
\fi

==> sections/unbounded_complexity_first_variant.tex <==
\section{Unbounded Communication Complexity Is Inherent In $\mathcal{PS}_{\delta}$}

In this section, we show that no Byzantine consensus protocol operating in $\mathcal{PS}_{\delta}$ exists with bounded communication complexity.
This result relies on the fact that no consensus protocol operating in $\mathcal{PS}_{\mathit{GST}, \delta}$ ensures bounded communication complexity before $\mathit{GST}$~\cite[Theorem 1]{spiegelman2021search}.

\begin{theorem} \label{theorem:unbounded_complexity_first_variant}
No Byzantine consensus protocol operating in $\mathcal{PS}_{\delta}$ exists that can tolerate a single failure and guarantee bounded communication complexity even in failure-free executions.
\end{theorem}
\begin{proof}
By contradiction, let there exist a Byzantine consensus protocol $\Pi$ operating in $\mathcal{PS}_{\delta}$ such that (1) $\Pi$ can tolerate a single failure, and (2) $\Pi$ has bounded communication complexity $X$ across all failure-free executions.
Next, we construct a Byzantine consensus protocol $\Pi'$ that operates in $\mathcal{PS}_{\mathit{GST}, \delta}$ by making $\Pi'$ behave in the same way as $\Pi$ in every execution.

$\Pi'$ solves the Byzantine consensus problem since $\Pi$ does so.
Moreover, for every failure-free execution $\alpha'$ of $\Pi'$, there exists the identical failure-free execution $\alpha$ of $\Pi$: if the maximum message delay in $\alpha'$ is $D$, then there exists the execution of $\Pi$ in which $\delta = D$ and all processes behave as in $\alpha'$.
Given that $\Pi$ has bounded communication complexity $X$ across all failure-free executions, $\Pi'$ has bounded communication complexity across all failure-free executions.
This contradicts Theorem 1 presented in~\cite{spiegelman2021search}, which concludes the theorem.
\end{proof}

\Cref{theorem:unbounded_complexity_first_variant} proves that it is inevitable to have unbounded communication complexity in solving the Byzantine consensus protocol in $\mathcal{PS}_{\delta}$.
Therefore, we turn our focus to the alternative variant $\mathcal{PS}_{\mathit{GST}, \delta}$ of the partially synchronous model.
\pierre{I think we have to stress, that it is not true if the unknown $\delta$ can be considered as a constant. Typically, the version of HotStuff where each correct process enters in a new view after timeout where the timer is increased exponentially has a communication complexity of $O((f+1+log_2(\delta))\cdot n)$ in $\mathcal{PS}_{\delta}$}



==> sections/vector_consensus.tex <==
\section{A reduction of vector consensus to consensus with external validity}

In this section, we show how to reduce the Byzantine Vector Consensus problem to the consensus with external validity. Such a reduction allows to solve all the variants of Byzantine consensus \cite{validity_paper}.

First, we present a straightforward composition to directly call \name where the possible inputs are vector of size $L = (n-t)(\kappa+\lambda)$, where $\lambda$ denotes the size of the proposal of one process.

Second, we take advantage of the particular structure of the vector validity property to propose a second algorithm that solves vector consensus with optimal linear latency and a communication complexity of $L \cdot n + \kappa \cdot n^3 \cdot log(n)$. 
Thus, for sufficiently large vectors (i.e. $\lambda = \Omega(\kappa n \mathit{log}(n))$), the result is optimal.

\subsection{Trivial Reduction}

\begin{algorithm} [t]
\caption{Trivial reduction from Vector Consensus to \name (for process $P_i$)}
\label{algorithm:trivial_vector_consensus}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em 
\textsc{Root}, \textbf{instance} $\mathit{root}$, where external validity predicate $\mathsf{Valid}()$ returns true only if the input is a vector of $(n-t)$ correctly signed proposal messages.

 \smallskip
\State \textbf{upon} $\mathsf{propose}(\mathit{proposal}_i)$: \BlueComment{start of the protocol} \label{line:start_trivial_vector_consensus}

\State \hskip2em \textbf{broadcast} $\langle \textsc{proposal}, \mathit{proposal}_i, \sigma_i(\mathit{proposal}_i) \rangle$ \label{line:bcast_proposal} 


%\smallskip
%\State \textbf{upon} reception of $\langle \textsc{Proposal}, \mathit{prop} \rangle$ from process $p_j$: 
%\State \hskip2em \textbf{send} $\langle \textsc{Observed}, \mathsf{Hash}(\mathit{prop})\rangle$ 

 \smallskip
\State \textbf{upon} reception of $\{\langle \textsc{proposal}, \mathit{prop}_j, \sigma_j \rangle \}_{j \in J}$ from a set $J$ of $n-t$ distinct processes:
\State \hskip2em \text{build} $\mathit{vector}_i$ as a vector of $(n-t)$ signed values from $\{\langle \textsc{proposal}, \mathit{prop}_j, \sigma_j \rangle \}_{j \in J}$
\State \hskip2em $\mathit{root}.\mathsf{propose}(\mathit{vector}_i)$

\smallskip
\State \textbf{upon} $\mathit{root}.\mathsf{decide}(\mathit{vec})$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{vec})$



\end{algorithmic}
\end{algorithm}

\subsection{Optimal Vector Consensus for very large inputs}

\begin{algorithm} [t]
\caption{Vector Consensus optimal for very large inputs (for process $P_i$)}
\label{algorithm:vector_consensus_for_very_large_inputs}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em \textsc{Spread}, \textbf{instance} $\mathit{spread}$ where external validity predicate $\mathsf{Valid}()$ returns true only if the input is a bit-mask with $n-t$ "1" digits accompanied with a vector of $(n-t)$ correctly signed proofs of observation.
\State \hskip2em \textsc{Quad}, \textbf{instance} $\mathit{quad}$
\State \hskip2em \textsc{Fix}, \textbf{instances} $\mathit{fix}_j$, $\forall j \in [0:n]$

 \smallskip
 
\State \textbf{Variables:}
%\State \hskip2em $\mathsf{Integer}$ $\mathit{counter\_fix} \gets 1$
\State \hskip2em $\mathsf{Map}(\mathsf{Processes} \rightarrow \mathsf{Proposals})$ $\mathit{proposals\_map}[]$
\State \hskip2em $\mathsf{Map}(\mathsf{Processes} \rightarrow \mathsf{Proofs\_Of\_Observation})$ $\mathit{proofs\_map}[]$
\State \hskip2em $\mathsf{Map}(\mathsf{Processes} \rightarrow \mathsf{Integers})$ $\mathit{observations\_map}[]$, initially $, \mathit{observations\_map}[j] = 0, \forall j \in [1:n]$

 \smallskip
\State \textbf{upon} $\mathsf{propose}(\mathit{proposal}_i)$: \BlueComment{start of the protocol} \label{line:start_trivial_vector_consensus}

\State \hskip2em \textbf{broadcast} $\langle \textsc{proposal}, \mathit{proposal}_i \rangle$ \label{line:bcast_proposal} 


\smallskip
\State \textbf{upon} reception of $\langle \textsc{Proposal}, \mathit{prop} \rangle$ from process $p_j$ for the first time: 
\State \hskip2em  $\mathit{observations\_map}[j] += 1$
\State \hskip2em \textbf{send} $\langle \textsc{Observed}, j, \mathsf{Hash}(\mathit{prop}), \sigma_i(\textsc{Observed}, j, \mathsf{Hash}(\mathit{prop}))\rangle$ 

\smallskip
\State \textbf{upon} reception of 
$\{ \langle \textsc{Observed}, i, \mathsf{Hash}(\mathit{proposal_i}), \sigma_j \rangle \}_{j \in J}$ from a set $J$ of $n-t$ processes:

\State \hskip2em $\sigma \gets \mathsf{combine}(\{\sigma_j\}_{j \in J})$

\State \hskip2em \textbf{broadcast} $\langle \textsc{Proof\_of\_Observation},  \mathsf{Hash}(\mathit{proposal_i}), \sigma \rangle$

\smallskip
\State \textbf{upon} reception of  $\langle \textsc{Proof\_of\_Observation},  h, \sigma \rangle$ from process $p_j$ for the first time:
\State \hskip2em  $\mathit{observations\_map}[j] += 1$
\State \hskip2em   $proofs\_map[j] := (h, \sigma)$

\smallskip
\State \textbf{upon} $\mathit{observations\_map}[j] == 2$, for every $j$ in a set $J$ of $n-t$ distinct processes
\State \hskip2em \text{build} $\mathit{input}_i := (\mathit{bit\_mask}_i, \mathit{proofs\_of\_observation}_i)$ where (1) $\forall j \in J, \mathit{bit\_mask}_i[j] = 1$ and $0$ otherwise, and (2)  $\forall j \in J, \mathit{proofs\_of\_observation}_i[j] = \mathit{proofs\_map}_i[j]$ and $\bot$ otherwise.
\State \hskip2em $\mathit{spread}.\mathsf{disseminate}(\mathit{input}_i)$

 
\smallskip
\State \textbf{upon} $\mathit{spread}.\mathsf{acquire}(h_i \in \mathsf{Hash\_Value}, \Sigma_i \in \mathsf{Proof})$: %\label{line:acquire}
\State \hskip2em \textbf{invoke} $\mathit{quad}.\mathsf{propose}(h_i, \Sigma_i)$ %\label{line:quad_propose}

\smallskip
\State \textbf{upon} $\mathit{quad}.\mathsf{decide}(h \in \mathsf{Hash\_Value}, \Sigma \in \mathsf{Proof})$: %\label{line:quad_decide}
\State \hskip2em $(\mathit{bit\_mask}, \mathit{proofs\_of\_observation}) \gets \mathit{input}$ s.t. $\mathsf{hash}(\mathit{input}) = h$ \BlueComment{can return $\bot$} %\label{line:check_obtained}
\State \hskip2em \textbf{invoke} $\mathit{fix}.\mathsf{input}(\mathit{input})$ %\label{line:vec_rec_input}

\smallskip
\State \textbf{upon} $\mathit{fix}.\mathsf{output}(\mathit{bit\_mask}', \mathit{proofs\_of\_observation}')$: %\label{line:vec_rec_output}


\State \hskip2em \textbf{for} $\mathsf{Integer}$ $j \in [1:n]$:
\State \hskip4em \textbf{if} $\mathit{bit\_mask}'[j] == 1$:
\State \hskip6em \textbf{invoke} $\mathit{fix}_{j}.\mathsf{input}(\mathit{proposals\_map}[j])$
%\State \hskip6em $\mathit{counter\_fix} \gets \mathit{counter\_fix} + 1$

\smallskip
\State \textbf{upon} $\mathit{fix}_j.\mathsf{output}(proposal_j)$ for every $j$ in a set $J$ of $n-t$ distinct processes:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{vec})$ where $\forall j \in j$, $\mathit{vec}[j] = proposal_j$
%\label{line:decide}


\end{algorithmic}
\end{algorithm}
